Comprehensive analysis of a dense sample of FRB 121102 bursts

We present an analysis of a densely repeating sample of bursts from the first repeating fast radio burst, FRB 121102. We reanalysed the data used by Gourdji et al. (2019) and detected 93 additional bursts using our single-pulse search pipeline. In total, we detected 133 bursts in three hours of data at a center frequency of 1.4 GHz using the Arecibo telescope, and develop robust modeling strategies to constrain the spectro-temporal properties of all the bursts in the sample. Most of the burst profiles show a scattering tail, and burst spectra are well modeled by a Gaussian with a median width of 230 MHz. We find a lack of emission below 1300 MHz, consistent with previous studies of FRB 121102. We also find that the peak of the log-normal distribution of wait times decreases from 207 s to 75 s using our larger sample of bursts, as compared to that of Gourdji et al. (2019). Our observations do not favor either Poissonian or Weibull distributions for the burst rate distribution. We searched for periodicity in the bursts using multiple techniques but did not detect any significant period. The cumulative burst energy distribution exhibits a broken power-law shape, with the lower and higher-energy slopes of $-0.4\pm0.1$ and $-1.8\pm0.2$, with the break at $(2.3\pm0.2)\times 10^{37}$ ergs. We provide our burst fitting routines as a python package BURSTFIT that can be used to model the spectrogram of any complex FRB or pulsar pulse using robust fitting techniques. All the other analysis scripts and results are publicly available.

==> Dense Sample of FRB121102 bursts/burst_table.tex <==
\startlongtable
\begin{deluxetable*}{lrrrrrrrrrrrrrrrrrrrrrr}
% \tablenum{1}
% \tablecaption{Astrometric Comparison \label{tab:astrometry}}
% \tablewidth{\linewidth}
\longrotatetable
% \tablehead{
% \colhead{Sr. No} & \multicolumn{2}{c}{Radio (J2000)} & \multicolumn{2}{c}{Optical (J2000)} & \multicolumn{2}{c}{Offset ($\arcsec$)}\\
% \colhead{} & \colhead{RA} & \colhead{DEC} & \colhead{RA} & \colhead{DEC} & \colhead{RA} & \colhead{DEC}}
\startdata
% \begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
% \rotatetable
% \toprule
% {} &  \$\textbackslash mu\_f\$ (MHz) &  upper error\$\textbackslash mu\_f\$ (MHz) &  lower error\$\textbackslash mu\_f\$ (MHz) &  \$\textbackslash sigma\_f\$ (MHz) &  upper error\$\textbackslash sigma\_f\$ (MHz) &  lower error\$\textbackslash sigma\_f\$ (MHz) &  \$S\$ (Jy ms) &  upper error\$S\$ (Jy ms) &  lower error\$S\$ (Jy ms) &  \$\textbackslash mu\_t\$ (ms) &  upper error\$\textbackslash mu\_t\$ (ms) &  lower error\$\textbackslash mu\_t\$ (ms) &  \$\textbackslash sigma\_t\$ (ms) &  upper error\$\textbackslash sigma\_t\$ (ms) &  lower error\$\textbackslash sigma\_t\$ (ms) &  \$\textbackslash tau\$ (ms) &  upper error\$\textbackslash tau\$ (ms) &  lower error\$\textbackslash tau\$ (ms) &  DM (pc cm\$\textasciicircum \{-3\}\$) &  upper errorDM (pc cm\$\textasciicircum \{-3\}\$) &  lower errorDM (pc cm\$\textasciicircum \{-3\}\$) &  comp\_num \\
% \midrule
0   &    3074.866031 &              2.235324e+02 &              5.558695e+02 &        549.818353 &                    83.033079 &                   111.124293 &     2.106578 &                3.684532 &                1.606049 &  57644.410073 &             3.601599e-09 &             4.030881e-09 &         1.066126 &                1.981733e-01 &                1.837101e-01 &     0.306613 &                0.169090 &                0.107359 &         563.878367 &                  1.017721e+00 &                  1.145842e+00 &         1 \\
1   &    2100.643913 &              9.380480e+02 &              1.617787e+03 &       2703.687541 &                   929.441672 &                  1238.095536 &     0.191984 &                0.048706 &                0.043850 &  57644.410158 &             4.198228e-09 &             4.241883e-09 &         0.661879 &                3.060655e-01 &                2.605480e-01 &     1.017467 &                0.422653 &                0.336476 &         562.082164 &                  7.254827e-01 &                  5.641742e-01 &         1 \\
2   &    3043.016847 &              2.468530e+02 &              5.551768e+02 &        651.601141 &                   126.841656 &                   138.216471 &     1.094175 &                1.498200 &                0.706197 &  57644.414124 &             4.416506e-09 &             3.798050e-09 &         1.002067 &                2.568850e-01 &                2.624549e-01 &     0.788696 &                0.357439 &                0.327918 &         567.458069 &                  9.422403e-01 &                  7.289469e-01 &         1 \\
3   &    1625.910301 &              1.097377e+01 &              1.112842e+01 &         81.941052 &                     8.484747 &                     7.630736 &     0.096903 &                0.010891 &                0.010307 &  57644.414475 &             7.814378e-09 &             7.028575e-09 &         1.441726 &                2.798057e-01 &                3.051317e-01 &     0.517916 &                0.289825 &                0.204750 &         562.070297 &                  2.744559e+00 &                  3.221510e+00 &         1 \\
4   &    1554.209322 &              1.074664e+01 &              1.097490e+01 &         96.109806 &                    12.949014 &                    10.630297 &     0.074124 &                0.007772 &                0.007439 &  57644.414879 &             4.285539e-09 &             4.634785e-09 &         0.846018 &                1.630260e-01 &                1.652373e-01 &     0.290967 &                0.183909 &                0.113241 &         560.324649 &                  9.282696e-01 &                  9.499163e-01 &         1 \\
5   &    3050.184527 &              2.119497e+02 &              2.986416e+02 &        450.459497 &                    63.929215 &                    76.973965 &    18.396136 &               16.474113 &               12.489799 &  57644.415378 &             9.298674e-09 &             1.039007e-08 &         1.931171 &                4.773695e-01 &                5.216117e-01 &     1.503911 &                1.301241 &                0.813175 &         568.583506 &                  3.498099e+00 &                  4.353664e+00 &         1 \\
6   &    1691.877912 &              1.267490e+01 &              9.384032e+00 &         88.653272 &                    15.908305 &                    11.837436 &     0.138823 &                0.011258 &                0.009906 &  57644.416315 &             4.503818e-09 &             4.867616e-09 &         1.487408 &                1.787762e-01 &                2.148986e-01 &     0.576520 &                0.318885 &                0.242019 &         571.851847 &                  1.470420e+00 &                  1.375934e+00 &         1 \\
7   &    1264.593451 &              1.026780e+01 &              9.957336e+00 &         67.355321 &                     8.601894 &                     7.840279 &     0.134822 &                0.020072 &                0.018831 &  57644.418307 &             6.829941e-08 &             8.276402e-08 &         2.951750 &                1.149607e+00 &                1.022370e+00 &     1.572956 &                0.599972 &                0.503402 &         562.018317 &                  5.858997e+00 &                  4.594390e+00 &         1 \\
8   &    3060.064914 &              2.280279e+02 &              5.946436e+02 &        510.421523 &                    64.135840 &                   111.276660 &     5.938947 &                9.144948 &                4.880618 &  57644.420509 &             4.096364e-09 &             4.336471e-09 &         1.189536 &                2.167979e-01 &                2.476828e-01 &     0.515828 &                0.287973 &                0.221253 &         570.290783 &                  1.691348e+00 &                  1.591659e+00 &         1 \\
9   &    2023.841501 &              9.894923e+02 &              1.662523e+03 &       2586.118211 &                  1009.910387 &                  1374.250034 &     0.151061 &                0.052290 &                0.041881 &  57644.421105 &             1.192529e-08 &             1.271837e-08 &         1.515181 &                5.527047e-01 &                5.232992e-01 &     0.739936 &                0.956501 &                0.352010 &         570.114031 &                  1.427338e+00 &                  1.930761e+00 &         1 \\
10  &    2855.697638 &              3.896675e+02 &              1.029775e+03 &       1048.190129 &                  1990.096884 &                   381.871492 &     0.233454 &                0.473724 &                0.079166 &  57644.427377 &             4.161848e-09 &             4.431058e-09 &         0.665876 &                2.837010e-01 &                3.299061e-01 &     0.591814 &                0.499724 &                0.308283 &         565.578180 &                  7.605473e-01 &                  5.649291e-01 &         1 \\
11  &    3103.820597 &              2.018182e+02 &              4.271795e+02 &        600.939265 &                   128.391839 &                   107.392819 &     2.734857 &                6.614627 &                1.852813 &  57644.427940 &             1.626177e-08 &             1.920125e-08 &         4.157687 &                8.739811e-01 &                9.919716e-01 &     1.820251 &                1.663655 &                0.835002 &         576.108744 &                  4.475180e+00 &                  5.135311e+00 &         1 \\
12  &    2991.434179 &              2.896015e+02 &              7.154517e+02 &        655.332362 &                   124.101717 &                   183.316387 &     1.338308 &                1.723632 &                0.936200 &  57644.428594 &             8.505594e-09 &             7.770723e-09 &         1.907938 &                4.269817e-01 &                4.178503e-01 &     1.526522 &                0.633527 &                0.631164 &         567.646156 &                  2.254513e+00 &                  2.149866e+00 &         1 \\
13  &    1698.759487 &              1.366499e+01 &              9.111177e+00 &         74.723176 &                    15.406403 &                     9.972977 &     0.089443 &                0.008710 &                0.007885 &  57644.430170 &             2.240995e-09 &             2.284651e-09 &         0.687118 &                1.052845e-01 &                1.099720e-01 &     0.332783 &                0.167763 &                0.144788 &         568.703039 &                  9.671064e-01 &                  9.771692e-01 &         1 \\
14  &    1753.113555 &              1.375950e+03 &              7.232516e+01 &        201.834574 &                   389.647488 &                    59.315807 &     0.161804 &                3.671485 &                0.031272 &  57644.430171 &             4.030881e-09 &             3.943569e-09 &         1.383852 &                1.743766e-01 &                1.975387e-01 &     0.661673 &                0.274440 &                0.258215 &         568.004469 &                  1.179303e+00 &                  1.158146e+00 &         1 \\
15  &    1469.638266 &              1.206921e+01 &              1.418449e+01 &        110.168894 &                    15.648925 &                    12.536650 &     0.096237 &                0.008865 &                0.008593 &  57644.431295 &             4.285539e-09 &             4.605681e-09 &         0.825079 &                1.765630e-01 &                1.691157e-01 &     0.489867 &                0.166650 &                0.169472 &         565.606060 &                  6.900090e-01 &                  6.774787e-01 &         1 \\
16  &    1344.471659 &              7.231304e+01 &              1.397881e+03 &       1123.000215 &                  2074.461619 &                   999.931723 &     0.172616 &                0.108263 &                0.085568 &  57644.432235 &             2.412708e-08 &             1.642184e-08 &         2.041703 &                9.811888e-01 &                6.821793e-01 &     1.074649 &                0.518550 &                0.405960 &         569.606721 &                  1.532792e+00 &                  2.172629e+00 &         1 \\
17  &    1753.873529 &              3.883385e+01 &              1.888832e+01 &         96.044583 &                    23.238518 &                    13.841937 &     0.136800 &                0.031607 &                0.015147 &  57644.432243 &             1.062290e-09 &             1.200533e-09 &         0.590009 &                4.580417e-02 &                4.600942e-02 &     0.157519 &                0.085570 &                0.052893 &         561.341086 &                  5.100551e-01 &                  5.005275e-01 &         1 \\
18  &    1682.086671 &              1.440497e+03 &              3.403930e+01 &        126.720043 &                   482.469828 &                    36.524709 &     0.062906 &                1.502574 &                0.013961 &  57644.434045 &             3.630703e-09 &             3.819878e-09 &         0.649565 &                1.837050e-01 &                1.652012e-01 &     0.415542 &                0.434776 &                0.227983 &         561.944971 &                  1.251747e+00 &                  3.338278e+00 &         1 \\
19  &    1438.436789 &              1.209237e+01 &              1.271892e+01 &         96.874532 &                    15.153189 &                    12.912619 &     0.120952 &                0.013904 &                0.013317 &  57644.436366 &             1.943408e-08 &             1.943408e-08 &         2.114945 &                5.862555e-01 &                5.351130e-01 &     1.171342 &                0.484130 &                0.424576 &         568.292911 &                  2.401008e+00 &                  2.515646e+00 &         1 \\
20  &    1501.654308 &              6.318258e+00 &              6.421393e+00 &        100.308781 &                     8.131903 &                     7.255264 &     0.191268 &                0.010069 &                0.009738 &  57644.438795 &             4.292815e-09 &             4.314643e-09 &         1.569189 &                1.411267e-01 &                1.505217e-01 &     0.466902 &                0.136887 &                0.131183 &         566.614957 &                  7.196468e-01 &                  7.352750e-01 &         1 \\
21  &    1410.170642 &              7.569828e+00 &              7.570620e+00 &         78.703681 &                     8.584276 &                     7.667938 &     0.136800 &                0.012764 &                0.011952 &  57644.438845 &             1.407898e-08 &             1.453009e-08 &         1.712679 &                2.874023e-01 &                3.804301e-01 &     0.645991 &                0.371919 &                0.266140 &         564.208575 &                  1.407150e+00 &                  1.391008e+00 &         1 \\
22  &    1476.816576 &              1.764255e+01 &              1.837630e+01 &        122.879736 &                    20.312368 &                    16.493155 &     0.077668 &                0.012491 &                0.010282 &  57644.439213 &             8.963980e-09 &             7.494236e-09 &         1.181245 &                3.026901e-01 &                3.555885e-01 &     0.593462 &                0.562631 &                0.291490 &         562.531953 &                  9.726264e-01 &                  1.335052e+00 &         1 \\
23  &    2559.531270 &              6.121318e+02 &              1.391842e+03 &       2052.859562 &                  1413.031171 &                  1089.324504 &     0.271982 &                0.101074 &                0.063633 &  57644.440689 &             5.151378e-09 &             5.631591e-09 &         1.276658 &                4.331835e-01 &                3.749133e-01 &     1.007187 &                0.405653 &                0.335115 &         567.032343 &                  8.125252e-01 &                  9.055199e-01 &         1 \\
24  &    1706.895880 &              5.255398e+00 &              4.676408e+00 &         60.556705 &                     5.794844 &                     4.920802 &     0.235009 &                0.012553 &                0.012401 &  57644.442998 &             5.384209e-09 &             5.777110e-09 &         2.754589 &                1.939485e-01 &                2.101955e-01 &     0.724094 &                0.360728 &                0.236483 &         575.259473 &                  2.618152e+00 &                  2.674777e+00 &         1 \\
25  &    3103.200327 &              1.946750e+02 &              4.059270e+02 &        474.923047 &                    65.301911 &                    88.311098 &    13.562077 &               23.919749 &               10.923801 &  57644.443589 &             1.658918e-08 &             2.646266e-08 &         2.964734 &                1.617569e+00 &                1.275405e+00 &     2.282858 &                1.555881 &                1.228661 &         574.414294 &                  1.111077e+01 &                  6.138218e+00 &         1 \\
26  &    1411.850547 &              2.385258e+01 &              1.689906e+01 &        133.180398 &                    28.234492 &                    15.536819 &     0.065361 &                0.006609 &                0.008498 &  57644.443590 &             3.012246e-09 &             3.965397e-09 &         0.582531 &                1.138658e-01 &                8.714409e-02 &     0.143780 &                0.100254 &                0.041402 &         562.804360 &                  4.703068e-01 &                  3.794158e-01 &         1 \\
27  &    1618.330258 &              1.839669e+01 &              1.603617e+01 &        110.114902 &                    20.796256 &                    15.157108 &     0.098552 &                0.014725 &                0.013936 &  57644.445225 &             8.025381e-09 &             6.562914e-09 &         0.908927 &                5.076986e-01 &                4.568527e-01 &     1.941624 &                0.717931 &                0.933281 &         567.429180 &                  1.547327e+00 &                  1.507595e+00 &         1 \\
28  &    1503.320019 &              1.389504e+01 &              1.780477e+01 &        126.004337 &                    12.821785 &                    12.278029 &     0.056761 &                0.009834 &                0.005824 &  57644.446788 &             1.025910e-09 &             1.738954e-09 &         0.210515 &                4.084608e-02 &                4.368951e-02 &     0.117640 &                0.130097 &                0.050336 &         560.903446 &                  1.483747e-01 &                  1.509667e-01 &         1 \\
29  &    1588.192968 &              1.037492e+01 &              1.034613e+01 &         81.401848 &                    10.775125 &                     9.141235 &     0.117638 &                0.017005 &                0.015048 &  57644.447568 &             8.825737e-09 &             7.421477e-09 &         1.132266 &                4.550410e-01 &                3.937062e-01 &     2.031254 &                0.766859 &                0.658937 &         559.847303 &                  2.627435e+00 &                  2.679809e+00 &         1 \\
30  &    1668.190100 &              1.470283e+01 &              1.166082e+01 &        108.039238 &                    18.422603 &                    15.684084 &     0.098879 &                0.008575 &                0.007991 &  57644.449916 &             2.844899e-09 &             2.881279e-09 &         0.933206 &                1.603030e-01 &                2.302788e-01 &     0.385870 &                0.233127 &                0.162074 &         565.960796 &                  7.981315e-01 &                  7.370288e-01 &         1 \\
31  &    1682.778949 &              1.212718e+01 &              9.065245e+00 &        123.545326 &                    15.464187 &                    12.451648 &     0.220447 &                0.012752 &                0.011042 &  57644.451605 &             1.367880e-09 &             1.295120e-09 &         0.794652 &                9.527094e-02 &                8.914728e-02 &     0.861114 &                0.114901 &                0.116967 &         568.158109 &                  4.500589e-01 &                  4.575727e-01 &         1 \\
32  &    3133.007516 &              1.752323e+02 &              3.555619e+02 &        521.759457 &                    53.669815 &                    71.453022 &    10.750999 &               12.859349 &                7.172429 &  57644.452390 &             6.199116e-09 &             5.813490e-09 &         1.820845 &                3.211144e-01 &                3.441520e-01 &     1.062797 &                0.519755 &                0.450985 &         568.780888 &                  2.326107e+00 &                  3.967006e+00 &         1 \\
33  &    1706.506824 &              1.486371e+03 &              5.735066e+01 &        161.988513 &                   474.968514 &                    74.460338 &     0.073680 &                1.805807 &                0.017110 &  57644.453937 &             4.474714e-09 &             3.812602e-09 &         0.868842 &                1.955563e-01 &                4.358830e-01 &     0.464707 &                0.410655 &                0.224231 &         562.476867 &                  1.387534e+00 &                  1.204624e+00 &         1 \\
34  &    1371.004537 &              2.147831e+00 &              2.229256e+00 &         61.489048 &                     2.308837 &                     2.215078 &     0.413836 &                0.012679 &                0.012414 &  57644.454477 &             8.207280e-09 &             8.236384e-09 &         2.765609 &                1.714455e-01 &                2.043305e-01 &     0.579716 &                0.140395 &                0.113697 &         569.599056 &                  8.297861e-01 &                  8.262580e-01 &         1 \\
35  &     894.507502 &              7.620895e+02 &              1.126316e+03 &       2011.222953 &                  1426.993479 &                  1715.332126 &     0.147564 &                0.044851 &                0.085532 &  57644.457883 &             3.143214e-09 &             2.633897e-09 &         0.501936 &                1.164454e-01 &                1.082587e-01 &     0.230207 &                0.135557 &                0.089106 &         561.936050 &                  2.577489e-01 &                  2.205913e-01 &         1 \\
36  &    1459.305290 &              1.016497e+01 &              1.073324e+01 &         85.536712 &                    10.825652 &                     9.552485 &     0.131336 &                0.015209 &                0.013934 &  57644.464763 &             1.196167e-08 &             1.225999e-08 &         1.335409 &                1.016914e+00 &                8.644005e-01 &     1.724340 &                0.599098 &                0.805386 &         561.484822 &                  2.394596e+00 &                  2.044029e+00 &         1 \\
37  &    2510.246818 &              6.473744e+02 &              9.160298e+02 &        951.881154 &                  1033.817204 &                   662.665551 &     0.315935 &                0.218037 &                0.191947 &  57644.465730 &             5.908078e-09 &             7.137714e-09 &         1.415205 &                5.608766e-01 &                3.817702e-01 &     1.156707 &                0.460134 &                0.407823 &         568.521350 &                  1.155807e+00 &                  1.180769e+00 &         1 \\
38  &    1667.343509 &              4.503356e+00 &              4.432376e+00 &         73.207001 &                     5.716007 &                     5.032887 &     0.184765 &                0.008873 &                0.008831 &  57644.466222 &             3.579771e-09 &             3.499736e-09 &         1.433698 &                1.459874e-01 &                1.585554e-01 &     0.631623 &                0.244238 &                0.239255 &         569.802339 &                  1.053614e+00 &                  1.049471e+00 &         1 \\
39  &    1715.831245 &              3.339547e+01 &              1.762622e+01 &        121.070355 &                    28.866351 &                    20.328101 &     0.191454 &                0.025641 &                0.016973 &  57644.468095 &             3.943569e-09 &             3.587047e-09 &         1.465745 &                2.426216e-01 &                2.234313e-01 &     1.124791 &                0.307505 &                0.343491 &         571.848392 &                  1.392233e+00 &                  1.385351e+00 &         1 \\
40  &    1648.709455 &              1.238575e+01 &              1.047486e+01 &         95.229489 &                    12.159934 &                     9.821915 &     0.130790 &                0.013169 &                0.011964 &  57644.474718 &             5.573384e-09 &             5.427864e-09 &         1.406831 &                2.669049e-01 &                2.417088e-01 &     1.285286 &                0.485314 &                0.460723 &         569.847221 &                  1.555281e+00 &                  1.583119e+00 &         1 \\
41  &    1706.126003 &              4.455174e+00 &              4.011692e+00 &         53.672923 &                     6.001413 &                     4.867634 &     0.161523 &                0.010557 &                0.010259 &  57644.477082 &             2.946763e-09 &             2.612069e-09 &         0.884572 &                1.603169e-01 &                1.382247e-01 &     0.909979 &                0.215300 &                0.222388 &         559.703915 &                  1.616269e+00 &                  1.655394e+00 &         1 \\
42  &    1530.213173 &              5.727281e+00 &              5.661187e+00 &        185.967267 &                     6.268319 &                     6.118243 &     0.253702 &                0.005759 &                0.005462 &  57645.411089 &             4.074536e-10 &             4.074536e-10 &         0.480743 &                2.506085e-02 &                2.396012e-02 &     0.209457 &                0.023042 &                0.024457 &         561.746352 &                  6.052966e-02 &                  6.053392e-02 &         1 \\
43  &    1462.010835 &              5.553152e+00 &              5.594528e+00 &         77.625610 &                     5.829904 &                     5.415621 &     0.129210 &                0.008103 &                0.007884 &  57645.411652 &             4.329195e-09 &             4.220055e-09 &         0.938840 &                1.489901e-01 &                1.358012e-01 &     0.410036 &                0.113743 &                0.119876 &         564.370351 &                  6.195938e-01 &                  6.505681e-01 &         1 \\
44  &    1536.584557 &              4.637798e+00 &              4.457538e+00 &         68.150290 &                     4.482496 &                     4.085008 &     0.201344 &                0.012168 &                0.011755 &  57645.411889 &             9.044015e-09 &             9.080395e-09 &         2.206685 &                3.529253e-01 &                3.360156e-01 &     1.098157 &                0.315794 &                0.345030 &         567.830593 &                  2.087382e+00 &                  2.019221e+00 &         1 \\
45  &    1437.894307 &              1.344831e+03 &              1.433164e+03 &       2809.123585 &                   854.915279 &                  1136.821635 &     0.250711 &                0.080272 &                0.067918 &  57645.412869 &             1.891021e-08 &             1.730950e-08 &         1.942670 &                2.359892e+00 &                9.978470e-01 &     2.483146 &                1.716731 &                1.152991 &         579.730888 &                  2.814247e+00 &                  1.336684e+01 &         1 \\
46  &    1574.834447 &              1.051695e+01 &              1.102502e+01 &        110.151733 &                    14.569998 &                    11.252887 &     0.119899 &                0.009656 &                0.009066 &  57645.413645 &             4.591129e-09 &             4.598405e-09 &         1.308066 &                2.061113e-01 &                2.173937e-01 &     0.611663 &                0.268956 &                0.237248 &         567.219651 &                  1.148594e+00 &                  1.250406e+00 &         1 \\
47  &    1276.268654 &              9.907018e+00 &              1.046554e+01 &         85.622207 &                    10.744013 &                     8.672704 &     0.103104 &                0.011392 &                0.010585 &  57645.416095 &             1.221633e-08 &             1.124135e-08 &         0.772538 &                2.422718e-01 &                2.069768e-01 &     0.601874 &                0.152525 &                0.139996 &         562.017081 &                  7.870831e-01 &                  8.581060e-01 &         1 \\
48  &    1824.658692 &              1.127025e+03 &              1.414468e+03 &       2631.968332 &                   983.372832 &                  1385.619418 &     0.315998 &                0.086042 &                0.093915 &  57645.416395 &             1.063017e-08 &             1.590524e-08 &         1.354395 &                4.831073e-01 &                4.717508e-01 &     2.528038 &                1.184442 &                1.253809 &         564.386687 &                  2.763047e+00 &                  1.763732e+00 &         1 \\
49  &    1549.302740 &              1.238233e+01 &              1.253089e+01 &        108.165411 &                    16.051127 &                    13.199135 &     0.091439 &                0.009100 &                0.008511 &  57645.416565 &             6.133632e-09 &             5.755282e-09 &         1.190103 &                2.234641e-01 &                2.328542e-01 &     0.572738 &                0.286101 &                0.236289 &         565.703772 &                  9.632887e-01 &                  1.132814e+00 &         1 \\
50  &    1438.283092 &              1.156853e+01 &              1.209166e+01 &        117.724997 &                    12.750942 &                    11.357021 &     0.104655 &                0.008589 &                0.008352 &  57645.417467 &             6.140908e-09 &             6.002665e-09 &         1.597562 &                1.640428e-01 &                1.502190e-01 &          NaN &                     NaN &                     NaN &         567.670017 &                  7.432870e-01 &                  7.140798e-01 &         1 \\
51  &    1639.949905 &              2.627778e+01 &              1.879937e+01 &        175.242092 &                    34.953992 &                    27.143575 &     0.099303 &                0.008999 &                0.007899 &  57645.417897 &             1.913577e-09 &             1.942681e-09 &         0.823244 &                1.052152e-01 &                1.134531e-01 &     0.313503 &                0.148577 &                0.118934 &         564.754956 &                  4.700210e-01 &                  5.049791e-01 &         1 \\
52  &    2078.748339 &              9.504298e+02 &              1.288309e+03 &       2389.310168 &                  1165.979362 &                  1376.413304 &     0.196102 &                0.051064 &                0.060172 &  57645.419006 &             9.793439e-09 &             5.733455e-09 &         0.976380 &                5.603939e-01 &                4.866207e-01 &     0.887142 &                0.412448 &                0.356371 &         567.938667 &                  9.387700e-01 &                  1.321105e+00 &         1 \\
53  &    1452.437833 &              1.565797e+01 &              1.373409e+01 &         84.319910 &                    13.939876 &                    12.536747 &     0.059015 &                0.008613 &                0.009182 &  57645.419207 &             1.065928e-08 &             8.789357e-09 &         0.732501 &                3.128089e-01 &                3.145160e-01 &     0.523796 &                0.284610 &                0.220513 &         564.482479 &                  1.319433e+00 &                  1.346727e+00 &         1 \\
54  &    3084.578024 &              2.173158e+02 &              4.594366e+02 &        636.750129 &                   146.021669 &                   116.310538 &     0.897362 &                1.698278 &                0.574115 &  57645.419896 &             3.594323e-09 &             3.739842e-09 &         0.793183 &                3.371007e-01 &                2.877284e-01 &     0.752933 &                0.389404 &                0.331647 &         563.805103 &                  1.354127e+00 &                  1.352878e+00 &         1 \\
55  &    1377.852703 &              4.584987e+00 &              4.450188e+00 &         78.105911 &                     4.514130 &                     4.201103 &     0.343787 &                0.018127 &                0.018032 &  57645.420266 &             9.742507e-09 &             8.847564e-09 &         0.997937 &                2.319654e-01 &                2.114472e-01 &     2.576255 &                0.240224 &                0.222771 &         561.077047 &                  8.693652e-01 &                  9.538554e-01 &         1 \\
56  &    3083.245091 &              2.168906e+02 &              4.631372e+02 &        655.946966 &                   239.483604 &                   138.808615 &     1.153999 &                3.418312 &                0.797813 &  57645.420600 &             1.075387e-08 &             7.064955e-09 &         1.165608 &                6.735023e-01 &                8.338094e-01 &     2.089366 &                1.334955 &                1.169319 &         558.973786 &                  1.589612e+00 &                  2.256962e+00 &         1 \\
57  &    3080.006672 &              2.201802e+02 &              4.673256e+02 &        616.137403 &                   135.897106 &                   115.434427 &     1.510880 &                2.934927 &                1.008181 &  57645.420680 &             7.355993e-09 &             5.951733e-09 &         1.541820 &                6.136190e-01 &                7.856533e-01 &     1.658819 &                0.833653 &                0.740008 &         574.831291 &                  2.985381e+00 &                  2.848148e+00 &         1 \\
58  &    3134.262020 &              1.766043e+02 &              3.970975e+02 &        522.748261 &                    95.546504 &                    87.129776 &     4.741475 &               12.315336 &                3.561078 &  57645.420752 &             5.755282e-09 &             6.642949e-09 &         1.156756 &                8.351653e-01 &                6.014175e-01 &     1.862063 &                0.695683 &                0.873280 &         551.223922 &                  1.070645e+01 &                  2.455613e+00 &         1 \\
59  &    2192.334917 &              8.460233e+02 &              1.430771e+03 &       2710.988090 &                   921.007274 &                  1205.982722 &     0.391624 &                0.068889 &                0.079138 &  57645.421284 &             3.819878e-09 &             4.110916e-09 &         0.901937 &                3.400151e-01 &                2.823390e-01 &     1.814649 &                0.345687 &                0.318261 &         567.621215 &                  9.428158e-01 &                  6.959242e-01 &         1 \\
60  &    1408.568517 &              1.358635e+01 &              3.520050e+02 &         93.912852 &                    22.657394 &                    13.599363 &     0.049803 &                0.111454 &                0.005826 &  57645.421291 &             5.304173e-09 &             4.562025e-09 &         0.424682 &                2.453251e-01 &                8.717474e-02 &     0.140114 &                0.415216 &                0.054827 &         561.627252 &                  5.751793e-01 &                  4.948632e-01 &         1 \\
61  &    1311.987182 &              5.233456e+00 &              5.437590e+00 &         51.087297 &                     6.497108 &                     5.735694 &     0.122126 &                0.010987 &                0.011020 &  57645.421613 &             1.741137e-08 &             2.342858e-08 &         1.293325 &                4.651924e-01 &                5.225449e-01 &     0.692962 &                0.228425 &                0.215155 &         565.730861 &                  2.180546e+00 &                  1.593501e+00 &         1 \\
62  &    1172.297671 &              1.718399e+01 &              3.618796e+01 &         77.921133 &                    35.690074 &                    13.469704 &     0.108801 &                0.027883 &                0.015008 &  57645.421848 &             1.339504e-08 &             1.594890e-08 &         0.874872 &                2.837906e-01 &                2.435208e-01 &     0.282655 &                0.141733 &                0.081908 &         562.413441 &                  7.209325e-01 &                  8.760608e-01 &         1 \\
63  &    1702.012160 &              4.147355e+00 &              4.029573e+00 &         56.897315 &                     5.611201 &                     4.808106 &     0.176938 &                0.011188 &                0.010390 &  57645.421872 &             3.383320e-09 &             3.368768e-09 &         1.192419 &                2.046551e-01 &                1.782679e-01 &     1.686745 &                0.290801 &                0.296226 &         568.033427 &                  2.209772e+00 &                  2.176216e+00 &         1 \\
64  &    1600.554398 &              7.277823e+00 &              7.744704e+00 &         80.877312 &                     8.360896 &                     7.439249 &     0.128628 &                0.009511 &                0.009663 &  57645.422455 &             3.034074e-09 &             2.939487e-09 &         0.522650 &                2.880950e-01 &                1.816306e-01 &     1.317777 &                0.235973 &                0.273817 &         564.441465 &                  1.034233e+00 &                  8.459594e-01 &         1 \\
65  &    1717.212820 &              3.944939e+02 &              1.466371e+01 &         64.744883 &                   306.212357 &                    24.613384 &     0.050891 &                0.099732 &                0.009647 &  57645.423009 &             5.820766e-09 &             7.166818e-09 &         0.783199 &                8.441999e-02 &                1.778067e-01 &     0.561716 &                0.120901 &                0.204573 &         563.165645 &                  8.251099e+00 &                  5.248670e+00 &         1 \\
66  &    3140.121855 &              1.739853e+02 &              3.583373e+02 &        575.510591 &                    62.726776 &                    72.848583 &     3.561114 &                3.929403 &                2.090306 &  57645.424146 &             2.328306e-09 &             2.393790e-09 &         1.325460 &                1.263448e-01 &                1.174236e-01 &          NaN &                     NaN &                     NaN &         569.170711 &                  6.610805e-01 &                  7.126597e-01 &         1 \\
67  &    2440.903225 &              7.032350e+02 &              1.295474e+03 &       1928.192994 &                  1504.101602 &                  1071.471827 &     0.148669 &                0.065564 &                0.044160 &  57645.424618 &             3.557943e-09 &             8.018105e-09 &         0.724224 &                3.268988e-01 &                3.202378e-01 &     0.410055 &                0.248994 &                0.173052 &         564.742043 &                  7.263469e-01 &                  4.873390e-01 &         1 \\
68  &    3035.226950 &              2.527243e+02 &              6.986593e+02 &        579.911391 &                   121.772213 &                   164.150448 &     1.435790 &                2.901608 &                1.135001 &  57645.425478 &             9.131327e-09 &             7.596100e-09 &         1.023308 &                7.743977e-01 &                6.473015e-01 &     1.671389 &                0.886643 &                0.884146 &         563.240428 &                  2.225785e+00 &                  2.611995e+00 &         1 \\
69  &    1550.128232 &              1.061614e+01 &              1.094080e+01 &         76.312315 &                    10.644020 &                     9.747604 &     0.067294 &                0.008933 &                0.008195 &  57645.426792 &             8.440111e-09 &             6.293703e-09 &         0.611601 &                3.742269e-01 &                3.479874e-01 &     0.852257 &                0.338342 &                0.339446 &         562.579231 &                  1.106607e+00 &                  1.367854e+00 &         1 \\
70  &    1756.117968 &              4.413000e+02 &              5.008304e+01 &        192.621544 &                   198.203931 &                    46.269040 &     0.201899 &                0.384048 &                0.030120 &  57645.426923 &             3.739842e-09 &             3.361492e-09 &         1.386565 &                2.039221e-01 &                1.968113e-01 &     0.919056 &                0.300820 &                0.320082 &         571.125090 &                  9.088061e-01 &                  9.496840e-01 &         1 \\
71  &    1479.240651 &              8.003131e+00 &              7.914794e+00 &        119.941071 &                     7.755897 &                     7.230659 &     0.183004 &                0.010539 &                0.010273 &  57645.428905 &             5.697075e-09 &             5.777110e-09 &         2.410542 &                1.651075e-01 &                1.543151e-01 &          NaN &                     NaN &                     NaN &         569.043835 &                  7.462246e-01 &                  7.601764e-01 &         1 \\
72  &    1418.436500 &              4.440680e+01 &              4.953823e+02 &        118.600756 &                  2788.936113 &                    33.871782 &     0.087619 &                0.108905 &                0.017107 &  57645.429900 &             1.824810e-08 &             1.992885e-08 &         2.356641 &                6.131942e-01 &                5.952364e-01 &     0.784561 &                0.601771 &                0.306418 &         564.685902 &                  2.002196e+00 &                  1.993743e+00 &         1 \\
73  &    1476.162699 &              9.002641e+00 &              9.484050e+00 &         80.936688 &                     9.701613 &                     8.042037 &     0.123489 &                0.012649 &                0.012447 &  57645.430345 &             1.758599e-08 &             1.777516e-08 &         3.114675 &                4.073805e-01 &                3.695247e-01 &          NaN &                     NaN &                     NaN &         571.912940 &                  2.322698e+00 &                  2.465981e+00 &         1 \\
74  &    1721.339203 &              4.106734e+00 &              4.125865e+00 &         38.667816 &                     5.548194 &                     4.296246 &     0.171942 &                0.017513 &                0.016620 &  57645.430448 &             1.109584e-08 &             1.077569e-08 &         2.637024 &                8.387583e-01 &                6.512917e-01 &     3.353441 &                1.081659 &                1.138255 &         575.227980 &                  1.037588e+01 &                  9.917636e+00 &         1 \\
75  &    3086.667479 &              2.142312e+02 &              6.056490e+02 &        498.722282 &                    58.931269 &                   116.565989 &     6.516961 &                9.992173 &                5.509438 &  57645.431306 &             3.936293e-09 &             4.074536e-09 &         1.131361 &                1.734233e-01 &                1.837735e-01 &     0.587614 &                0.369326 &                0.275993 &         565.224818 &                  1.693125e+00 &                  3.897621e+00 &         1 \\
76  &    1692.871860 &              1.146298e+01 &              8.444990e+00 &         91.646632 &                    20.251070 &                    14.123113 &     0.095355 &                0.007254 &                0.006691 &  57645.431478 &             1.549779e-09 &             1.673470e-09 &         0.687566 &                7.854712e-02 &                7.777064e-02 &     0.219348 &                0.120278 &                0.082055 &         563.513258 &                  5.723842e-01 &                  5.491343e-01 &         1 \\
77  &    1561.692073 &              1.303021e+03 &              1.516138e+03 &       2832.011301 &                   831.532584 &                  1141.303726 &     0.201720 &                0.056948 &                0.052034 &  57645.432545 &             1.397711e-08 &             1.694571e-08 &         2.051485 &                8.049102e-01 &                8.878593e-01 &     0.915765 &                0.577661 &                0.343658 &         564.615438 &                  1.756645e+00 &                  1.456396e+00 &         1 \\
78  &    2886.980686 &              3.641469e+02 &              7.808702e+02 &        804.979024 &                   544.515982 &                   229.019999 &     0.280421 &                0.421296 &                0.137702 &  57645.433087 &             3.761670e-09 &             2.626621e-09 &         0.571785 &                3.737512e-01 &                3.931337e-01 &     0.963890 &                0.351383 &                0.383984 &         562.421584 &                  8.836179e-01 &                  5.134757e-01 &         1 \\
79  &    1667.327751 &              7.314304e+00 &              7.260931e+00 &         66.812593 &                     7.870246 &                     6.665671 &     0.093815 &                0.009607 &                0.008978 &  57645.434330 &             5.187758e-09 &             5.158654e-09 &         1.097623 &                2.287482e-01 &                2.309131e-01 &     0.703326 &                0.305770 &                0.306397 &         559.497769 &                  2.217240e+00 &                  2.023495e+00 &         1 \\
80  &    1601.963477 &              1.277694e+03 &              1.503042e+03 &       2819.214819 &                   836.621500 &                  1140.150497 &     0.131291 &                0.031019 &                0.030013 &  57645.440067 &             4.110916e-09 &             4.380126e-09 &         0.799775 &                2.307853e-01 &                2.377410e-01 &     0.299180 &                0.231177 &                0.122822 &         565.776251 &                  3.511802e-01 &                  3.632283e-01 &         1 \\
81  &    1687.768615 &              3.686276e+00 &              3.711556e+00 &         62.058151 &                     5.302570 &                     4.672710 &     0.154459 &                0.007777 &                0.007417 &  57645.440815 &             2.095476e-09 &             1.920853e-09 &         0.955599 &                1.111654e-01 &                1.192815e-01 &     0.481068 &                0.181199 &                0.188627 &         566.927119 &                  9.709680e-01 &                  1.006559e+00 &         1 \\
82  &    2012.812267 &              1.159713e+03 &              3.333432e+02 &        341.179486 &                   297.910241 &                   208.973441 &     0.244789 &                2.660051 &                0.134871 &  57645.442100 &             7.275958e-09 &             8.316420e-09 &         2.108279 &                4.172739e-01 &                3.788079e-01 &     0.825778 &                0.628305 &                0.367181 &         563.539968 &                  1.801948e+00 &                  2.112779e+00 &         1 \\
83  &    1469.085028 &              1.273257e+01 &              1.454663e+01 &         87.190691 &                    13.747526 &                    12.566362 &     0.084329 &                0.011578 &                0.010206 &  57645.442633 &             1.178705e-08 &             1.447188e-08 &         1.371368 &                3.061635e-01 &                3.487483e-01 &     0.647338 &                0.481793 &                0.291887 &         562.454932 &                  1.480708e+00 &                  1.395851e+00 &         1 \\
84  &    1671.039915 &              1.113620e+01 &              9.895401e+00 &        107.110278 &                    22.607508 &                    16.549133 &     0.095381 &                0.007534 &                0.006896 &  57645.444481 &             1.644366e-09 &             1.477019e-09 &         0.509815 &                1.027496e-01 &                8.774176e-02 &     0.459451 &                0.122129 &                0.134779 &         565.370224 &                  5.232001e-01 &                  4.982806e-01 &         1 \\
85  &    1480.346346 &              7.227445e+00 &              7.577572e+00 &         96.554595 &                    10.365147 &                     9.423247 &     0.161804 &                0.010538 &                0.010504 &  57645.444919 &             7.028575e-09 &             6.861228e-09 &         1.975454 &                2.235563e-01 &                2.246655e-01 &     0.517873 &                0.195281 &                0.147700 &         565.842807 &                  1.073413e+00 &                  1.137353e+00 &         1 \\
86  &    2780.502613 &              2.500543e+02 &              9.995685e+02 &        368.180339 &                    71.826952 &                   256.126994 &    10.415885 &               12.013203 &               10.275748 &  57645.445443 &             5.129550e-09 &             4.314643e-09 &         1.216438 &                2.802890e-01 &                2.696089e-01 &     0.872813 &                0.391531 &                0.373970 &         560.861657 &                  2.640700e+00 &                  2.211774e+00 &         1 \\
87  &    1487.773014 &              3.733883e+00 &              3.807171e+00 &         83.027930 &                     3.672020 &                     3.557013 &     0.141104 &                0.005723 &                0.005553 &  57645.448803 &             1.833541e-09 &             1.782610e-09 &         0.660208 &                3.446256e-02 &                3.341631e-02 &          NaN &                     NaN &                     NaN &         561.071367 &                  2.577523e-01 &                  2.595136e-01 &         1 \\
88  &    1460.096696 &              4.741149e+00 &              4.849608e+00 &         87.196937 &                     5.090963 &                     4.727356 &     0.236683 &                0.011926 &                0.011599 &  57645.449987 &             7.625204e-09 &             7.741619e-09 &         2.807350 &                1.910706e-01 &                1.701220e-01 &          NaN &                     NaN &                     NaN &         568.064149 &                  1.011289e+00 &                  1.005672e+00 &         1 \\
89  &    1468.658600 &              5.720229e+00 &              5.866068e+00 &         57.790404 &                     6.713271 &                     5.931767 &     0.109160 &                0.009557 &                0.008956 &  57645.451990 &             1.255103e-08 &             1.350418e-08 &         1.582808 &                2.202104e-01 &                2.275626e-01 &     0.451615 &                0.196799 &                0.145180 &         563.310760 &                  2.019741e+00 &                  1.876428e+00 &         1 \\
90  &    1441.750838 &              4.282132e+00 &              4.574567e+00 &         67.521331 &                     4.491711 &                     4.331328 &     0.142443 &                0.008169 &                0.007853 &  57645.453426 &             4.227331e-09 &             4.125468e-09 &         0.591629 &                8.301529e-02 &                7.364113e-02 &     0.396539 &                0.067631 &                0.063572 &         563.089528 &                  5.543240e-01 &                  5.741314e-01 &         1 \\
91  &    1699.312840 &              3.779977e+00 &              3.635988e+00 &         68.370255 &                     5.971942 &                     5.062319 &     0.286153 &                0.011905 &                0.011530 &  57645.453639 &             3.652531e-09 &             4.183676e-09 &         2.483659 &                1.467723e-01 &                1.608944e-01 &     0.630212 &                0.290123 &                0.196818 &         569.028554 &                  1.614829e+00 &                  1.599067e+00 &         1 \\
92  &    1569.933745 &              1.656213e+01 &              1.757871e+01 &        109.003850 &                    24.912993 &                    18.667109 &     0.072980 &                0.010282 &                0.010060 &  57645.453640 &             3.063178e-09 &             2.954039e-09 &         0.254396 &                1.648204e-01 &                1.264443e-01 &     1.411967 &                0.330369 &                0.274767 &         566.533113 &                  6.728565e-01 &                  7.640658e-01 &         1 \\
93  &    1725.024812 &              2.628075e+01 &              1.346705e+01 &         94.709930 &                    24.883944 &                    15.333299 &     0.186049 &                0.025653 &                0.018184 &  57645.454258 &             6.330083e-09 &             6.744813e-09 &         2.268887 &                3.416549e-01 &                3.406638e-01 &     0.905585 &                0.561563 &                0.394976 &         569.292928 &                  2.536592e+00 &                  2.556439e+00 &         1 \\
94  &    1576.744880 &              2.445421e+01 &              2.342648e+01 &        131.079919 &                    34.460174 &                    21.362071 &     0.100828 &                0.016266 &                0.013884 &  57645.457361 &             1.077569e-08 &             1.268927e-08 &         1.766544 &                8.953911e-01 &                7.852575e-01 &     1.844145 &                0.846138 &                0.810665 &         562.614312 &                  2.848020e+00 &                  2.809466e+00 &         1 \\
95  &    1577.552397 &              2.501565e+01 &              2.304966e+01 &        131.336004 &                    33.983069 &                    21.485348 &     0.101176 &                0.016160 &                0.013928 &  57645.457361 &             1.077569e-08 &             1.252920e-08 &         1.749081 &                9.040648e-01 &                7.903621e-01 &     1.846625 &                0.854186 &                0.816190 &         562.558001 &                  2.875217e+00 &                  2.784554e+00 &         1 \\
96  &    1667.386391 &              6.334383e+01 &              2.475809e+01 &        167.055473 &                    63.947137 &                    29.376005 &     0.205133 &                0.035931 &                0.021680 &  57645.458536 &             5.202310e-09 &             5.988113e-09 &         1.227376 &                3.951017e-01 &                3.237630e-01 &     2.575740 &                0.480812 &                0.453056 &         568.800809 &                  1.775660e+00 &                  1.623564e+00 &         1 \\
97  &    1685.621021 &              1.041330e+03 &              2.542183e+01 &        127.486496 &                   380.916953 &                    29.005063 &     0.093946 &                0.867994 &                0.012945 &  57645.459103 &             5.231414e-09 &             6.089977e-09 &         0.776975 &                2.793762e-01 &                4.525519e-01 &     1.165137 &                0.478490 &                0.433633 &         566.379933 &                  1.821465e+00 &                  1.802054e+00 &         1 \\
98  &    1404.767162 &              4.246737e+00 &              4.179313e+00 &         70.790571 &                     5.255382 &                     5.022942 &     0.219696 &                0.011578 &                0.010933 &  57645.462107 &             9.313226e-09 &             9.473297e-09 &         2.271639 &                2.147267e-01 &                2.379545e-01 &     0.538642 &                0.175217 &                0.134516 &         564.708325 &                  1.027707e+00 &                  1.050837e+00 &         1 \\
99  &    1564.161526 &              1.490550e+01 &              1.520809e+01 &        145.437862 &                    22.784740 &                    19.037722 &     0.093862 &                0.008250 &                0.007726 &  57645.464053 &             2.924935e-09 &             2.830348e-09 &         0.962076 &                1.890339e-01 &                1.963829e-01 &     0.451252 &                0.204958 &                0.185094 &         565.313351 &                  5.314845e-01 &                  5.523109e-01 &         1 \\
100 &    1595.749037 &              1.446407e+01 &              1.439002e+01 &        144.104436 &                    20.923474 &                    17.430612 &     0.121358 &                0.009528 &                0.008974 &  57645.464189 &             3.703462e-09 &             3.710738e-09 &         1.244406 &                2.045444e-01 &                1.971149e-01 &     0.676185 &                0.225945 &                0.226959 &         564.424909 &                  7.548122e-01 &                  7.685186e-01 &         1 \\
101 &    1595.063990 &              1.187663e+03 &              5.748560e+01 &        225.987576 &                  2384.186386 &                    92.760915 &     0.074805 &                0.127797 &                0.019338 &  57645.464504 &             4.802132e-09 &             6.883056e-09 &         0.898964 &                3.659809e-01 &                5.131654e-01 &     0.852086 &                0.559731 &                0.426303 &         567.123622 &                  1.694344e+00 &                  1.933640e+00 &         1 \\
102 &    1966.525128 &              1.061649e+03 &              9.618014e+02 &       1970.737810 &                  1485.777072 &                  1706.845842 &     0.187780 &                0.064073 &                0.107246 &  57645.465133 &             6.883056e-09 &             6.592018e-09 &         0.759331 &                3.598308e-01 &                3.950503e-01 &     1.244785 &                0.584390 &                0.528811 &         566.009529 &                  1.935865e+00 &                  7.164909e-01 &         1 \\
103 &    1480.411416 &              1.132439e+03 &              1.328713e+03 &       2685.980603 &                   940.372315 &                  1535.483238 &     0.249445 &                0.052931 &                0.089305 &  57645.466101 &             5.602487e-09 &             5.507900e-09 &         1.120910 &                2.250362e-01 &                2.290677e-01 &     0.853499 &                0.299941 &                0.270546 &         567.002550 &                  7.252529e-01 &                  9.279284e-01 &         1 \\
104 &    1707.801832 &              1.378613e+03 &              1.532414e+01 &         89.118709 &                   445.440501 &                    26.610952 &     0.105725 &                4.564796 &                0.015450 &  57645.466380 &             4.751200e-09 &             4.474714e-09 &         1.019786 &                3.128417e-01 &                2.776730e-01 &     1.281008 &                0.418171 &                0.443851 &         573.207006 &                  1.998230e+00 &                  3.367167e+00 &         1 \\
105 &    1901.548147 &              1.082015e+03 &              1.418163e+03 &       2541.995267 &                  1043.979742 &                  1358.104203 &     0.184137 &                0.048689 &                0.052797 &  57645.468339 &             9.880750e-09 &             1.043372e-08 &         1.383362 &                3.962387e-01 &                3.757498e-01 &     0.587090 &                0.361215 &                0.248660 &         565.521749 &                  1.024529e+00 &                  8.451510e-01 &         1 \\
106 &    1461.076106 &              1.262501e+01 &              1.295560e+01 &         85.245144 &                    11.894901 &                    10.166661 &     0.084625 &                0.011527 &                0.010755 &  57645.472362 &             1.103763e-08 &             9.844371e-09 &         1.110243 &                3.610032e-01 &                3.288853e-01 &     0.749826 &                0.341681 &                0.296195 &         563.598782 &                  1.437588e+00 &                  1.675788e+00 &         1 \\
107 &    1715.320616 &              7.813194e+01 &              1.576692e+01 &         95.379198 &                    69.513985 &                    20.686252 &     0.089624 &                0.032942 &                0.010734 &  57645.474139 &             2.663000e-09 &             2.604793e-09 &         0.690257 &                1.376523e-01 &                1.483729e-01 &     0.395660 &                0.193369 &                0.175950 &         561.227089 &                  1.142549e+00 &                  1.243536e+00 &         1 \\
108 &    1739.638221 &              1.846262e+02 &              4.982098e+01 &        229.296500 &                   107.793207 &                    42.555969 &     0.220687 &                0.104798 &                0.027413 &  57645.474448 &             3.637979e-09 &             3.630703e-09 &         1.703164 &                2.005568e-01 &                2.041107e-01 &     0.692113 &                0.267207 &                0.251620 &         570.610408 &                  7.343792e-01 &                  7.044133e-01 &         1 \\
109 &    1146.748385 &              3.366306e+02 &              1.402431e+03 &       1268.197550 &                  1953.434745 &                  1118.096950 &     0.086795 &                0.132006 &                0.043727 &  57644.409674 &             2.612069e-09 &             3.556488e-08 &         0.315255 &                1.403977e+00 &                1.723546e-01 &     0.312379 &                0.722624 &                0.137925 &         564.674681 &                  1.460324e+00 &                  4.092879e-01 &         1 \\
110 &    2944.173246 &              3.174336e+02 &              5.864031e+02 &        751.069969 &                   291.263416 &                   192.031255 &     0.570043 &                0.746781 &                0.291921 &  57644.409674 &             3.885361e-09 &             2.830348e-09 &         0.369395 &                2.490799e-01 &                2.281785e-01 &     1.314203 &                0.653280 &                0.679797 &         566.808964 &                  7.847368e-01 &                  8.769143e-01 &         2 \\
111 &    1417.185501 &              3.884362e+00 &              4.659306e+00 &        101.935080 &                     4.761585 &                     4.084079 &     0.325358 &                0.026361 &                0.022544 &  57644.411072 &             8.731149e-10 &             9.677024e-10 &         0.567630 &                2.700489e-02 &                2.445215e-02 &          NaN &                     NaN &                     NaN &         560.936842 &                  1.509793e-01 &                  1.044998e-01 &         1 \\
112 &    1393.269756 &              7.335915e+00 &              6.580718e+00 &        182.694545 &                     7.031695 &                     7.319653 &     0.467987 &                0.023566 &                0.028527 &  57644.411072 &             1.367880e-09 &             1.506123e-09 &         1.086188 &                3.465937e-02 &                3.873258e-02 &          NaN &                     NaN &                     NaN &         562.334956 &                  2.126868e-01 &                  1.065625e-01 &         2 \\
113 &    3075.140018 &              2.057216e+02 &              3.100464e+02 &        432.303770 &                    64.815598 &                    80.479943 &    13.452290 &               16.886532 &               10.182305 &  57644.412240 &             5.980837e-09 &             3.921741e-09 &         0.658892 &                3.373955e-01 &                3.599354e-01 &     0.768458 &                0.438102 &                0.388007 &         568.514000 &                  2.818942e+00 &                  2.877411e+00 &         1 \\
114 &    1463.742248 &              1.658431e+01 &              1.993333e+01 &         92.445449 &                    26.420576 &                    16.196889 &     0.088688 &                0.014082 &                0.013198 &  57644.412240 &             1.666194e-08 &             2.434535e-08 &         1.938207 &                8.501248e-01 &                9.716448e-01 &     1.217235 &                0.557406 &                0.491706 &         568.620714 &                  3.480267e+00 &                  2.489991e+00 &         2 \\
115 &    1571.805268 &              1.256349e+03 &              1.318236e+03 &       2666.550717 &                   958.678509 &                  1462.952833 &     0.123130 &                0.034537 &                0.042314 &  57644.418309 &             2.692104e-09 &             2.044544e-09 &         0.229590 &                1.847969e-01 &                1.297846e-01 &     0.668237 &                0.224315 &                0.184028 &         569.377581 &                  3.826299e-01 &                  5.025129e-01 &         1 \\
116 &    1545.045684 &              1.218522e+01 &              1.231491e+01 &         79.220876 &                    12.863110 &                    10.388883 &     0.070604 &                0.012331 &                0.009849 &  57644.418309 &             6.701157e-09 &             8.214556e-09 &         0.893852 &                2.734982e-01 &                3.360123e-01 &     0.801977 &                0.525646 &                0.426765 &         564.836206 &                  1.702351e+00 &                  1.442758e+00 &         2 \\
117 &    2930.107980 &              3.016985e+02 &              1.238434e+03 &        554.920581 &                  2490.569338 &                   124.141388 &     1.279397 &               14.634899 &                1.104360 &  57644.464507 &             4.205504e-09 &             1.034641e-08 &         0.439924 &                3.701301e-01 &                2.670467e-01 &     0.746212 &                0.558681 &                0.348719 &         565.336884 &                  3.505241e+00 &                  2.291546e+00 &         1 \\
118 &      42.021699 &              1.287440e+03 &              5.240128e+02 &        546.664913 &                   543.613741 &                   417.624036 &     0.680933 &               26.226319 &                0.604790 &  57644.464508 &             3.983223e-07 &             2.954766e-08 &         0.850994 &                3.160707e+00 &                5.917550e-01 &     0.739398 &                3.571361 &                0.399140 &         564.241525 &                  1.454247e+02 &                  1.787667e+02 &         2 \\
119 &    1662.786572 &              1.499023e+01 &              1.138795e+01 &        135.639202 &                    17.252011 &                    14.123430 &     0.489810 &                0.029315 &                0.025773 &  57644.464759 &             1.374428e-08 &             1.445005e-08 &         8.336477 &                4.778664e-01 &                5.268128e-01 &     2.020312 &                0.734084 &                0.560803 &         568.020948 &                  3.895079e+00 &                  3.654518e+00 &         1 \\
120 &    2408.606972 &              7.136065e+02 &              1.401466e+03 &       2188.401233 &                  1310.395809 &                  1218.531156 &     0.156516 &                0.046767 &                0.038592 &  57644.464760 &             1.382432e-09 &             1.200533e-09 &         0.185676 &                1.360711e-01 &                1.089510e-01 &     0.552460 &                0.157799 &                0.147933 &         561.288155 &                  2.687443e-01 &                  1.567342e-01 &         2 \\
121 &    2269.117500 &              9.391856e+02 &              6.164983e+02 &        480.669655 &                   257.208127 &                   340.492478 &     0.360950 &                1.617964 &                0.245056 &  57645.412282 &             4.707545e-09 &             7.203198e-09 &         0.923363 &                5.702387e-01 &                5.487713e-01 &     2.507109 &                0.622974 &                0.509643 &         561.226766 &                  2.176630e+00 &                  1.712408e+00 &         1 \\
122 &    2952.955595 &              2.777356e+02 &              9.628994e+02 &        444.308412 &                    83.254251 &                   219.514873 &     4.070263 &                6.121378 &                3.929537 &  57645.412282 &             4.198228e-09 &             4.321919e-09 &         0.806123 &                1.742116e-01 &                1.409412e-01 &     0.328451 &                0.252032 &                0.159700 &         566.470854 &                  1.882520e+00 &                  1.738781e+00 &         2 \\
123 &    1458.599318 &              1.644780e+01 &              1.490549e+01 &        129.153657 &                    20.637665 &                    18.109982 &     0.109650 &                0.011784 &                0.011503 &  57645.427339 &             9.611540e-09 &             8.738425e-09 &         2.425962 &                3.816166e-01 &                3.478435e-01 &          NaN &                     NaN &                     NaN &         561.417523 &                  1.233301e+00 &                  1.519567e+00 &         1 \\
124 &    1894.125125 &              1.118269e+03 &              1.280715e+03 &       2407.093455 &                  1151.324507 &                  1543.217255 &     0.170886 &                0.059182 &                0.063451 &  57645.427339 &             7.021299e-09 &             6.853952e-09 &         0.742815 &                4.118685e-01 &                3.354176e-01 &     0.999411 &                0.666392 &                0.459778 &         561.185124 &                  1.673829e+00 &                  3.835765e+00 &         2 \\
125 &    1619.393987 &              1.350507e+01 &              1.339468e+01 &        122.792391 &                    19.610028 &                    15.503931 &     0.125426 &                0.011404 &                0.010902 &  57645.430623 &             6.621121e-09 &             6.606570e-09 &         1.728894 &                2.681988e-01 &                2.719235e-01 &     0.833053 &                0.394873 &                0.348592 &         564.472772 &                  1.957007e+00 &                  1.993448e+00 &         1 \\
126 &    1591.185401 &              8.643409e+00 &              8.622450e+00 &        106.246000 &                     9.690033 &                     8.605795 &     0.125593 &                0.008276 &                0.008099 &  57645.430622 &             2.961315e-09 &             3.063178e-09 &         1.175100 &                1.450225e-01 &                1.730884e-01 &     0.425621 &                0.207728 &                0.160133 &         565.279441 &                  7.579312e-01 &                  8.540979e-01 &         2 \\
127 &    1321.229539 &              2.350287e+00 &              2.591631e+00 &        178.089922 &                     2.393557 &                     2.192153 &     1.727278 &                0.016501 &                0.015766 &  57645.460053 &             3.565219e-10 &             3.710738e-10 &         0.950290 &                1.873480e-02 &                1.945944e-02 &     0.359745 &                0.015174 &                0.014633 &         561.979243 &                  2.641728e-02 &                  2.541783e-02 &         1 \\
128 &    1612.124857 &              1.982065e+00 &              1.948663e+00 &         89.558102 &                     1.776238 &                     1.794595 &     0.394344 &                0.007414 &                0.007265 &  57645.460053 &             9.968062e-10 &             9.968062e-10 &         0.817610 &                3.670013e-02 &                3.776732e-02 &     0.246287 &                0.058706 &                0.065201 &         562.082991 &                  1.678879e-01 &                  1.549020e-01 &         2 \\
129 &    1180.703156 &              8.763004e+00 &              1.092836e+01 &         92.749644 &                     8.914158 &                     7.840191 &     0.347690 &                0.025733 &                0.022437 &  57645.460053 &             4.161848e-09 &             4.198228e-09 &         1.221049 &                8.947771e-02 &                7.062640e-02 &          NaN &                     NaN &                     NaN &         561.591314 &                  2.490463e-01 &                  2.528331e-01 &         3 \\
130 &    1510.117308 &              2.071554e+01 &              2.071554e+01 &        133.202939 &                    21.510060 &                    21.510060 &     0.042229 &                0.002325 &                0.002434 &  57645.442000 &             2.823072e-09 &             2.830348e-09 &         0.867898 &                2.088193e-02 &                2.088193e-02 &          NaN &                     NaN &                     NaN &           0.548700 &                  8.577100e-03 &                  8.577100e-03 &         1 \\
131 &    1670.266306 &              1.956107e+01 &              1.956107e+01 &         83.299578 &                    17.949689 &                    17.949689 &     0.038362 &                0.002933 &                0.004161 &  57644.430170 &             1.120497e-09 &             1.120497e-09 &         0.022502 &                5.245603e-02 &                5.245603e-02 &     1.184573 &                0.279687 &                0.279687 &         563.027933 &                  4.789163e-01 &                  4.789163e-01 &         1 \\
132 &    1597.958397 &              2.164807e+07 &              2.164807e+07 &        119.798457 &                815228.179720 &                815228.179720 &     0.046001 &              673.184372 &                     NaN &  57644.471178 &             1.926910e-02 &             1.926910e-02 &         0.000061 &                9.463654e+02 &                9.463654e+02 &     0.915043 &                0.194515 &                0.194515 &         564.219980 &                  1.263647e+06 &                  1.263647e+06 &         1 \\
133 &    1325.047334 &              2.504631e+01 &              2.504631e+01 &        155.341622 &                    23.929991 &                    23.929991 &     0.105346 &                0.009151 &                0.010004 &  57644.427210 &             1.682929e-08 &             1.682201e-08 &         1.862538 &                7.574584e-01 &                7.574584e-01 &     1.629269 &                0.519683 &                0.519683 &         563.619089 &                  1.438477e+00 &                  1.438477e+00 &         1 \\
134 &    1201.746909 &              9.566596e+00 &              9.566596e+00 &         50.113890 &                     9.582602 &                     9.582602 &     0.043276 &                0.002974 &                0.003165 &  57644.409568 &             1.412263e-08 &             1.411536e-08 &         1.352605 &                4.683643e-02 &                4.683643e-02 &          NaN &                     NaN &                     NaN &           0.914970 &                  1.221681e-01 &                  1.221681e-01 &         1 \\
135 &    1693.821972 &              1.558198e+01 &              1.558198e+01 &         87.565055 &                    17.957167 &                    17.957167 &     0.087618 &                0.007053 &                0.007637 &  57645.462556 &             6.097252e-09 &             6.104528e-09 &         1.141818 &                3.995876e-01 &                3.995876e-01 &     2.020600 &                0.633372 &                0.633372 &         567.138100 &                  2.866725e+00 &                  2.866725e+00 &         1 \\
136 &    1378.895119 &              1.347993e+00 &              1.347993e+00 &         30.835678 &                     1.344029 &                     1.344029 &     0.400891 &                0.010523 &                0.010797 &  57644.447727 &             1.723674e-08 &             1.722947e-08 &         0.783981 &                1.713189e-01 &                1.713189e-01 &     3.046816 &                0.209123 &                0.209123 &         558.887533 &                  1.729084e+00 &                  1.729084e+00 &         1 \\
137 &    1526.468893 &              2.556739e+01 &              2.556739e+01 &        136.077031 &                    27.045035 &                    27.045035 &     0.046438 &                0.003060 &                0.003225 &  57644.426304 &             4.481990e-09 &             4.474714e-09 &         1.484517 &                9.867641e-02 &                9.867641e-02 &          NaN &                     NaN &                     NaN &           0.942675 &                  3.104992e-03 &                  3.104992e-03 &         1 \\
138 &    1428.074624 &              1.130210e+01 &              1.130210e+01 &         75.406334 &                     9.214344 &                     9.214344 &     0.076461 &                0.001212 &                0.001677 &  57644.414472 &             1.908484e-08 &             1.908484e-08 &         1.978465 &                6.320594e-01 &                6.320594e-01 &     0.374386 &                0.569700 &                0.569700 &         564.319250 &                  2.101098e+00 &                  2.101098e+00 &         1 \\
139 &    1460.908407 &              6.399049e+01 &              6.399049e+01 &         93.404158 &                    18.294892 &                    18.294892 &     0.067000 &                0.073632 &                0.089068 &  57645.442741 &             1.317312e-07 &             1.317239e-07 &         0.007516 &                2.039446e+00 &                2.039446e+00 &     2.072048 &                0.536759 &                0.536759 &         568.595557 &                  7.617052e+00 &                  7.617052e+00 &         1 \\
140 &    1619.713506 &              1.240310e+01 &              1.240310e+01 &        103.789170 &                    13.706690 &                    13.706690 &     0.102777 &                0.006001 &                0.006370 &  57645.451201 &             7.850758e-09 &             7.843482e-09 &         1.720296 &                4.327078e-01 &                4.327078e-01 &     1.324193 &                0.543372 &                0.543372 &         561.153658 &                  1.922735e+00 &                  1.922735e+00 &         1 \\
141 &    1296.131947 &              2.760286e+01 &              2.760286e+01 &        144.063844 &                    25.669848 &                    25.669848 &     0.098513 &                0.011069 &                0.012383 &  57645.426747 &             1.644366e-09 &             1.637090e-09 &         0.014181 &                5.825055e-02 &                5.825055e-02 &     1.727077 &                0.438122 &                0.438122 &         566.064993 &                  1.382615e-01 &                  1.382615e-01 &         1 \\
142 &    1393.789741 &              1.799780e+06 &              1.799780e+06 &         52.886662 &                 34154.830232 &                 34154.830232 &     0.022488 &              397.050200 &                     NaN &  57645.426747 &             1.238509e-02 &             1.238509e-02 &         0.000018 &                1.200626e+06 &                1.200626e+06 &     1.195847 &                0.802779 &                0.802779 &         569.703900 &                  8.121671e+05 &                  8.121671e+05 &         2 \\
143 &    1475.052916 &              4.450116e+01 &              4.450116e+01 &        261.543218 &                    62.152991 &                    62.152991 &     0.075349 &                0.006574 &                0.007136 &  57645.454493 &             9.094947e-10 &             9.022187e-10 &         0.049879 &                6.966984e-02 &                6.966984e-02 &     1.394718 &                0.272584 &                0.272584 &         565.674154 &                  1.528706e-01 &                  1.528706e-01 &         1 \\
144 &    1558.745535 &              3.399751e+01 &              3.399751e+01 &        212.380150 &                    44.927400 &                    44.927400 &     0.089441 &                0.006933 &                0.007452 &  57644.408907 &             1.418812e-09 &             1.418812e-09 &         0.001231 &                1.571490e-02 &                1.571490e-02 &     1.947448 &                0.337326 &                0.337326 &         565.336150 &                  4.118707e-01 &                  4.118707e-01 &         1 \\
\enddata
\end{deluxetable*}


==> Dense Sample of FRB121102 bursts/fitting_stuff.tex <==
check in final table: 
cand_tstart_57645.409861111111_tcand_1086.2000000_dm_562.05600_snr_6.40849_fit_results.png
cand_tstart_57644.407719907409_tcand_4864.6800000_dm_568.56200_snr_6.72464_fit_results.png
cand_tstart_57645.409861111111_tcand_159.4330000_dm_558.83100_snr_7.95436_fit_results.png

Good: 
1 comp:
cand_tstart_57645.409861111111_tcand_1719.8800000_dm_581.80000_snr_7.37079_fit_results.png
cand_tstart_57645.409861111111_tcand_3732.4400000_dm_565.30000_snr_6.74773_fit_results.png
cand_tstart_57645.409861111111_tcand_3589.8600000_dm_565.30000_snr_7.05175_fit_results.png
cand_tstart_57645.409861111111_tcand_965.5470000_dm_571.84300_snr_8.61639_fit_results.png
cand_tstart_57645.409861111111_tcand_644.5610000_dm_565.30000_snr_11.90090_fit_results.png

2 comp: 
cand_tstart_57645.409861111111_tcand_1743.9100000_dm_558.83100_snr_13.70630_fit_results.png


==> Dense Sample of FRB121102 bursts/small_table.tex <==
\begin{deluxetable*}{llllllll}%cccccccc}
\tablecaption{Properties of the first 10 bursts. See Appendix for the full table.}
\label{tab:small_table}
\tablehead{\colhead{Burst}\tablenotemark{a} & \colhead{$\mu_f$} & \colhead{$\sigma_f$} & \colhead{$S$} & \colhead{$\mu_t$\tablenotemark{b}} & \colhead{$\sigma_t$ } & \colhead{$\tau$\tablenotemark{c}} & \colhead{DM}\\
\colhead{ID} & \colhead{(MHz)} & \colhead{(MHz)} & \colhead{(Jy ms)} & \colhead{(MJD)} & \colhead{(ms)} & \colhead{(ms)} & \colhead{(pc cm$^{-3}$)}}
\startdata
B1$*$ & $1560^{+30}_{-30}$ & $210^{+40}_{-40}$ & $0.09^{+0.02}_{-0.02}$ & 57644.408906976(1) & $0.0^{+0.02}_{-0.02}$ & $1.9^{+0.3}_{-0.3}$ & $565.3^{+0.4}_{-0.4}$\\
B2$*$ & $1200^{+10}_{-10}$ & $50^{+10}_{-10}$ & $0.043^{+0.007}_{-0.007}$ & 57644.40956768(1) & $1.35^{+0.05}_{-0.05}$ & - & $562.4^{+0.8}_{-0.8}$\\
B3.1$\dagger$ & $2900^{+300}_{-600}$ & $800^{+300}_{-200}$ & $0.6^{+0.7}_{-0.3}$ & 57644.409673699(3) & $0.4^{+0.2}_{-0.2}$ & $1.3^{+0.7}_{-0.7}$ & $566.8^{+0.8}_{-0.9}$\\
B3.2$\dagger$ & $1100^{+300}_{-1400}$ & $1000^{+2000}_{-1000}$ & $0.09^{+0.13}_{-0.04}$ & 57644.40967384(2) & $0.3^{+1.4}_{-0.2}$ & $0.3^{+0.7}_{-0.1}$ & $564.7^{+1.5}_{-0.4}$\\
B4$\dagger$ & $3100^{+200}_{-600}$ & $550^{+80}_{-110}$ & $2^{+4}_{-2}$ & 57644.410072889(4) & $1.1^{+0.2}_{-0.2}$ & $0.3^{+0.2}_{-0.1}$ & $564^{+1}_{-1}$\\
B5$\dagger$ & $2100^{+900}_{-1600}$ & $2700^{+900}_{-1200}$ & $0.19^{+0.05}_{-0.04}$ & 57644.410157834(4) & $0.7^{+0.3}_{-0.3}$ & $1.0^{+0.4}_{-0.3}$ & $562.1^{+0.7}_{-0.6}$\\
B6.1 & $1393^{+7}_{-7}$ & $183^{+7}_{-7}$ & $0.47^{+0.02}_{-0.03}$ & 57644.411071954(1) & $1.09^{+0.03}_{-0.04}$ & - & $562.3^{+0.2}_{-0.1}$\\
B6.2 & $1417^{+4}_{-5}$ & $102^{+5}_{-4}$ & $0.33^{+0.03}_{-0.02}$ & 57644.4110719755(9) & $0.57^{+0.03}_{-0.02}$ & - & $560.9^{+0.2}_{-0.1}$\\
B7.1$\dagger$ & $3100^{+200}_{-300}$ & $430^{+60}_{-80}$ & $10^{+20}_{-10}$ & 57644.412240214(5) & $0.7^{+0.3}_{-0.4}$ & $0.8^{+0.4}_{-0.4}$ & $569^{+3}_{-3}$\\
B7.2$\dagger$ & $1460^{+20}_{-20}$ & $90^{+30}_{-20}$ & $0.09^{+0.01}_{-0.01}$ & 57644.41224043(2) & $1.9^{+0.9}_{-1.0}$ & $1.2^{+0.6}_{-0.5}$ & $569^{+3}_{-2}$\\
B8$\dagger$ & $3000^{+200}_{-600}$ & $700^{+100}_{-100}$ & $1.1^{+1.5}_{-0.7}$ & 57644.414123628(4) & $1.0^{+0.3}_{-0.3}$ & $0.8^{+0.4}_{-0.3}$ & $567.5^{+0.9}_{-0.7}$\\
B9$*$ & $1430^{+10}_{-10}$ & $75^{+9}_{-9}$ & $0.076^{+0.003}_{-0.003}$ & 57644.41447161(2) & $2.0^{+0.6}_{-0.6}$ & $0.4^{+0.6}_{-0.6}$ & $564^{+2}_{-2}$\\
B10 & $1630^{+10}_{-10}$ & $82^{+8}_{-8}$ & $0.1^{+0.01}_{-0.01}$ & 57644.414475391(7) & $1.4^{+0.3}_{-0.3}$ & $0.5^{+0.3}_{-0.2}$ & $562^{+3}_{-3}$\\
\enddata
\tablecomments{1$\sigma$ errors on the fits are shown on superscript and subscript of each value in the table. For $\mu_t$, the error on the last significant digit is shown in parenthesis.}
\tablenotetext{a}{Burst IDs are chronological. Individual component number (N) for multi-component bursts are appended to the burst IDs. Bursts modeled only using \texttt{curve\_fit} are marked with $*$. Note that the errors on these bursts could be unreliable and may be either under or over-estimated}. Bursts that extend beyond the observable bandwidth can also have unreliable estimates of spectra parameters and fluence (see Section~\ref{sec:fitcaveats}). We mark those bursts with $\dagger$ to indicate that their fluence and spectra parameters could be unconstrained. 
\tablenotetext{b}{$\mu_t$ is the mean of the pulse profile in units of MJD. This can be considered as the arrival time of the pulse. It is referenced to the solar system barycenter, after correcting to infinite frequency using a DM of 560.5\dmunits.}
\tablenotetext{c}{$\tau$ is referred to 1~GHz.}
% \tablenotetext{c}{Bursts which did not require $\tau$ during modeling are }
\end{deluxetable*}


==> Dense Sample of FRB121102 bursts/table.tex <==
\startlongtable
\begin{deluxetable*}{llllllll}
\tablecaption{Properties of all the bursts presented in this analysis.}
\label{tab:large_table}
\tablehead{\colhead{Burst}\tablenotemark{a} & \colhead{$\mu_f$} & \colhead{$\sigma_f$} & \colhead{$S$} & \colhead{$\mu_t$\tablenotemark{b}} & \colhead{$\sigma_t$ } & \colhead{$\tau$\tablenotemark{c}} & \colhead{DM}\\
\colhead{ID} & \colhead{(MHz)} & \colhead{(MHz)} & \colhead{(Jy ms)} & \colhead{(MJD)} & \colhead{(ms)} & \colhead{(ms)} & \colhead{(pc cm$^{-3}$)}}
\startdata
B1$*$ & $1560^{+30}_{-30}$ & $210^{+40}_{-40}$ & $0.09^{+0.02}_{-0.02}$ & 57644.408906976(1) & $0.0^{+0.02}_{-0.02}$ & $1.9^{+0.3}_{-0.3}$ & $565.3^{+0.4}_{-0.4}$\\
B2$*$ & $1200^{+10}_{-10}$ & $50^{+10}_{-10}$ & $0.043^{+0.007}_{-0.007}$ & 57644.40956768(1) & $1.35^{+0.05}_{-0.05}$ & - & $562.4^{+0.8}_{-0.8}$\\
B3.1$\dagger$ & $2900^{+300}_{-600}$ & $800^{+300}_{-200}$ & $0.6^{+0.7}_{-0.3}$ & 57644.409673699(3) & $0.4^{+0.2}_{-0.2}$ & $1.3^{+0.7}_{-0.7}$ & $566.8^{+0.8}_{-0.9}$\\
B3.2$\dagger$ & $1100^{+300}_{-1400}$ & $1000^{+2000}_{-1000}$ & $0.09^{+0.13}_{-0.04}$ & 57644.40967384(2) & $0.3^{+1.4}_{-0.2}$ & $0.3^{+0.7}_{-0.1}$ & $564.7^{+1.5}_{-0.4}$\\
B4$\dagger$ & $3100^{+200}_{-600}$ & $550^{+80}_{-110}$ & $2^{+4}_{-2}$ & 57644.410072889(4) & $1.1^{+0.2}_{-0.2}$ & $0.3^{+0.2}_{-0.1}$ & $564^{+1}_{-1}$\\
B5$\dagger$ & $2100^{+900}_{-1600}$ & $2700^{+900}_{-1200}$ & $0.19^{+0.05}_{-0.04}$ & 57644.410157834(4) & $0.7^{+0.3}_{-0.3}$ & $1.0^{+0.4}_{-0.3}$ & $562.1^{+0.7}_{-0.6}$\\
B6.1 & $1393^{+7}_{-7}$ & $183^{+7}_{-7}$ & $0.47^{+0.02}_{-0.03}$ & 57644.411071954(1) & $1.09^{+0.03}_{-0.04}$ & - & $562.3^{+0.2}_{-0.1}$\\
B6.2 & $1417^{+4}_{-5}$ & $102^{+5}_{-4}$ & $0.33^{+0.03}_{-0.02}$ & 57644.4110719755(9) & $0.57^{+0.03}_{-0.02}$ & - & $560.9^{+0.2}_{-0.1}$\\
B7.1$\dagger$ & $3100^{+200}_{-300}$ & $430^{+60}_{-80}$ & $10^{+20}_{-10}$ & 57644.412240214(5) & $0.7^{+0.3}_{-0.4}$ & $0.8^{+0.4}_{-0.4}$ & $569^{+3}_{-3}$\\
B7.2$\dagger$ & $1460^{+20}_{-20}$ & $90^{+30}_{-20}$ & $0.09^{+0.01}_{-0.01}$ & 57644.41224043(2) & $1.9^{+0.9}_{-1.0}$ & $1.2^{+0.6}_{-0.5}$ & $569^{+3}_{-2}$\\
B8$\dagger$ & $3000^{+200}_{-600}$ & $700^{+100}_{-100}$ & $1.1^{+1.5}_{-0.7}$ & 57644.414123628(4) & $1.0^{+0.3}_{-0.3}$ & $0.8^{+0.4}_{-0.3}$ & $567.5^{+0.9}_{-0.7}$\\
B9$*$ & $1430^{+10}_{-10}$ & $75^{+9}_{-9}$ & $0.076^{+0.003}_{-0.003}$ & 57644.41447161(2) & $2.0^{+0.6}_{-0.6}$ & $0.4^{+0.6}_{-0.6}$ & $564^{+2}_{-2}$\\
B10 & $1630^{+10}_{-10}$ & $82^{+8}_{-8}$ & $0.1^{+0.01}_{-0.01}$ & 57644.414475391(7) & $1.4^{+0.3}_{-0.3}$ & $0.5^{+0.3}_{-0.2}$ & $562^{+3}_{-3}$\\
B11 & $1550^{+10}_{-10}$ & $100^{+10}_{-10}$ & $0.074^{+0.008}_{-0.007}$ & 57644.414878803(4) & $0.8^{+0.2}_{-0.2}$ & $0.3^{+0.2}_{-0.1}$ & $560.3^{+0.9}_{-0.9}$\\
B12 & $3100^{+200}_{-300}$ & $450^{+60}_{-80}$ & $20^{+20}_{-10}$ & 57644.41537809(1) & $1.9^{+0.5}_{-0.5}$ & $1.5^{+1.3}_{-0.8}$ & $569^{+3}_{-4}$\\
B13 & $1692^{+13}_{-9}$ & $90^{+20}_{-10}$ & $0.14^{+0.01}_{-0.01}$ & 57644.416314736(5) & $1.5^{+0.2}_{-0.2}$ & $0.6^{+0.3}_{-0.2}$ & $572^{+1}_{-1}$\\
B14 & $1260^{+10}_{-10}$ & $67^{+9}_{-8}$ & $0.13^{+0.02}_{-0.02}$ & 57644.41830674(8) & $3^{+1}_{-1}$ & $1.6^{+0.6}_{-0.5}$ & $562^{+6}_{-5}$\\
B15.1$\dagger$ & $1550^{+10}_{-10}$ & $80^{+10}_{-10}$ & $0.07^{+0.01}_{-0.01}$ & 57644.418309206(7) & $0.9^{+0.3}_{-0.3}$ & $0.8^{+0.5}_{-0.4}$ & $565^{+2}_{-1}$\\
B15.2$\dagger$ & $2000^{+1000}_{-1000}$ & $3000^{+1000}_{-1000}$ & $0.12^{+0.03}_{-0.04}$ & 57644.418309273(2) & $0.2^{+0.2}_{-0.1}$ & $0.7^{+0.2}_{-0.2}$ & $569.4^{+0.4}_{-0.5}$\\
B16$\dagger$ & $3100^{+200}_{-600}$ & $510^{+60}_{-110}$ & $6^{+9}_{-5}$ & 57644.420508580(4) & $1.2^{+0.2}_{-0.2}$ & $0.5^{+0.3}_{-0.2}$ & $570^{+2}_{-2}$\\
B17 & $2000^{+1000}_{-2000}$ & $3000^{+1000}_{-1000}$ & $0.15^{+0.05}_{-0.04}$ & 57644.42110545(1) & $1.5^{+0.6}_{-0.5}$ & $0.7^{+1.0}_{-0.4}$ & $570^{+1}_{-2}$\\
B18$*$ & $1530^{+30}_{-30}$ & $140^{+30}_{-30}$ & $0.046^{+0.008}_{-0.008}$ & 57644.426303862(4) & $1.5^{+0.1}_{-0.1}$ & - & $564.8^{+0.8}_{-0.8}$\\
B19$*$ & $1330^{+30}_{-30}$ & $160^{+20}_{-20}$ & $0.11^{+0.02}_{-0.02}$ & 57644.42721003(2) & $1.9^{+0.8}_{-0.8}$ & $1.6^{+0.5}_{-0.5}$ & $564^{+1}_{-1}$\\
B20$\dagger$ & $2900^{+400}_{-1000}$ & $1000^{+2000}_{-400}$ & $0.23^{+0.47}_{-0.08}$ & 57644.427376859(4) & $0.7^{+0.3}_{-0.3}$ & $0.6^{+0.5}_{-0.3}$ & $565.6^{+0.8}_{-0.6}$\\
B21$\dagger$ & $3100^{+200}_{-400}$ & $600^{+100}_{-100}$ & $3^{+7}_{-2}$ & 57644.42794036(2) & $4.2^{+0.9}_{-1.0}$ & $1.8^{+1.7}_{-0.8}$ & $576^{+4}_{-5}$\\
B22$\dagger$ & $3000^{+300}_{-700}$ & $700^{+100}_{-200}$ & $1.3^{+1.7}_{-0.9}$ & 57644.428593784(8) & $1.9^{+0.4}_{-0.4}$ & $1.5^{+0.6}_{-0.6}$ & $568^{+2}_{-2}$\\
B23 & $1699^{+14}_{-9}$ & $70^{+20}_{-10}$ & $0.089^{+0.009}_{-0.008}$ & 57644.430170170(2) & $0.7^{+0.1}_{-0.1}$ & $0.3^{+0.2}_{-0.1}$ & $569.0^{+1.0}_{-1.0}$\\
B24$*$ & $1670^{+20}_{-20}$ & $80^{+20}_{-20}$ & $0.0384^{+0.0007}_{-0.0007}$ & 57644.430170303(1) & $0.02^{+0.05}_{-0.05}$ & $1.2^{+0.3}_{-0.3}$ & $563.0^{+0.5}_{-0.5}$\\
B25 & $1750^{+1380}_{-70}$ & $200^{+390}_{-60}$ & $0.16^{+3.67}_{-0.03}$ & 57644.430171419(4) & $1.4^{+0.2}_{-0.2}$ & $0.7^{+0.3}_{-0.3}$ & $568^{+1}_{-1}$\\
B26 & $1470^{+10}_{-10}$ & $110^{+20}_{-10}$ & $0.096^{+0.009}_{-0.009}$ & 57644.431295361(4) & $0.8^{+0.2}_{-0.2}$ & $0.5^{+0.2}_{-0.2}$ & $565.6^{+0.7}_{-0.7}$\\
B27 & $1340^{+70}_{-1400}$ & $1000^{+2000}_{-1000}$ & $0.17^{+0.11}_{-0.09}$ & 57644.43223490(2) & $2.0^{+1.0}_{-0.7}$ & $1.1^{+0.5}_{-0.4}$ & $570^{+2}_{-2}$\\
B28 & $1750^{+40}_{-20}$ & $100^{+20}_{-10}$ & $0.14^{+0.03}_{-0.02}$ & 57644.432242722(1) & $0.59^{+0.05}_{-0.05}$ & $0.16^{+0.09}_{-0.05}$ & $561.3^{+0.5}_{-0.5}$\\
B29 & $1680^{+1440}_{-30}$ & $130^{+480}_{-40}$ & $0.06^{+1.5}_{-0.01}$ & 57644.434045197(4) & $0.6^{+0.2}_{-0.2}$ & $0.4^{+0.4}_{-0.2}$ & $562^{+1}_{-3}$\\
B30 & $1440^{+10}_{-10}$ & $100^{+20}_{-10}$ & $0.12^{+0.01}_{-0.01}$ & 57644.43636575(2) & $2.1^{+0.6}_{-0.5}$ & $1.2^{+0.5}_{-0.4}$ & $568^{+2}_{-3}$\\
B31 & $1502^{+6}_{-6}$ & $100^{+8}_{-7}$ & $0.19^{+0.01}_{-0.01}$ & 57644.438794966(4) & $1.6^{+0.1}_{-0.2}$ & $0.5^{+0.1}_{-0.1}$ & $566.6^{+0.7}_{-0.7}$\\
B32 & $1410^{+8}_{-8}$ & $79^{+9}_{-8}$ & $0.14^{+0.01}_{-0.01}$ & 57644.43884518(1) & $1.7^{+0.3}_{-0.4}$ & $0.6^{+0.4}_{-0.3}$ & $564^{+1}_{-1}$\\
B33 & $1480^{+20}_{-20}$ & $120^{+20}_{-20}$ & $0.08^{+0.01}_{-0.01}$ & 57644.439212855(8) & $1.2^{+0.3}_{-0.4}$ & $0.6^{+0.6}_{-0.3}$ & $563.0^{+1.0}_{-1.0}$\\
B34$\dagger$ & $2600^{+600}_{-1400}$ & $2000^{+1000}_{-1000}$ & $0.27^{+0.1}_{-0.06}$ & 57644.440688613(5) & $1.3^{+0.4}_{-0.4}$ & $1.0^{+0.4}_{-0.3}$ & $567.0^{+0.8}_{-0.9}$\\
B35 & $1707^{+5}_{-5}$ & $61^{+6}_{-5}$ & $0.24^{+0.01}_{-0.01}$ & 57644.442997729(6) & $2.8^{+0.2}_{-0.2}$ & $0.7^{+0.4}_{-0.2}$ & $575^{+3}_{-3}$\\
B36$\dagger$ & $3100^{+200}_{-400}$ & $470^{+70}_{-90}$ & $10^{+20}_{-10}$ & 57644.44358918(2) & $3^{+2}_{-1}$ & $2^{+2}_{-1}$ & $574^{+11}_{-6}$\\
B37 & $1410^{+20}_{-20}$ & $130^{+30}_{-20}$ & $0.065^{+0.007}_{-0.008}$ & 57644.443590029(3) & $0.58^{+0.11}_{-0.09}$ & $0.14^{+0.1}_{-0.04}$ & $562.8^{+0.5}_{-0.4}$\\
B38 & $1620^{+20}_{-20}$ & $110^{+20}_{-20}$ & $0.1^{+0.01}_{-0.01}$ & 57644.445225058(7) & $0.9^{+0.5}_{-0.5}$ & $1.9^{+0.7}_{-0.9}$ & $567^{+2}_{-2}$\\
B39 & $1500^{+10}_{-20}$ & $130^{+10}_{-10}$ & $0.057^{+0.01}_{-0.006}$ & 57644.446788124(1) & $0.21^{+0.04}_{-0.04}$ & $0.12^{+0.13}_{-0.05}$ & $560.9^{+0.1}_{-0.2}$\\
B40 & $1590^{+10}_{-10}$ & $81^{+11}_{-9}$ & $0.12^{+0.02}_{-0.02}$ & 57644.447567822(8) & $1.1^{+0.5}_{-0.4}$ & $2.0^{+0.8}_{-0.7}$ & $560^{+3}_{-3}$\\
B41$*$ & $1379^{+1}_{-1}$ & $31^{+1}_{-1}$ & $0.4^{+0.02}_{-0.02}$ & 57644.44772750(2) & $0.8^{+0.2}_{-0.2}$ & $3.0^{+0.2}_{-0.2}$ & $559^{+2}_{-2}$\\
B42 & $1670^{+10}_{-10}$ & $110^{+20}_{-20}$ & $0.099^{+0.009}_{-0.008}$ & 57644.449915568(3) & $0.9^{+0.2}_{-0.2}$ & $0.4^{+0.2}_{-0.2}$ & $566.0^{+0.8}_{-0.7}$\\
B43 & $1683^{+12}_{-9}$ & $120^{+20}_{-10}$ & $0.22^{+0.01}_{-0.01}$ & 57644.451605444(1) & $0.79^{+0.1}_{-0.09}$ & $0.9^{+0.1}_{-0.1}$ & $568.2^{+0.5}_{-0.5}$\\
B44$\dagger$ & $3100^{+200}_{-400}$ & $520^{+50}_{-70}$ & $11^{+13}_{-7}$ & 57644.452389712(6) & $1.8^{+0.3}_{-0.3}$ & $1.1^{+0.5}_{-0.5}$ & $569^{+2}_{-4}$\\
B45 & $1710^{+1490}_{-60}$ & $160^{+470}_{-70}$ & $0.07^{+1.81}_{-0.02}$ & 57644.453937473(4) & $0.9^{+0.2}_{-0.4}$ & $0.5^{+0.4}_{-0.2}$ & $562^{+1}_{-1}$\\
B46 & $1371^{+2}_{-2}$ & $61^{+2}_{-2}$ & $0.41^{+0.01}_{-0.01}$ & 57644.454477404(8) & $2.8^{+0.2}_{-0.2}$ & $0.6^{+0.1}_{-0.1}$ & $569.6^{+0.8}_{-0.8}$\\
B47 & $900^{+800}_{-1100}$ & $2000^{+1000}_{-2000}$ & $0.15^{+0.04}_{-0.09}$ & 57644.457883227(3) & $0.5^{+0.1}_{-0.1}$ & $0.23^{+0.14}_{-0.09}$ & $561.9^{+0.3}_{-0.2}$\\
B48.1$\dagger$ & $2900^{+300}_{-1200}$ & $600^{+2500}_{-100}$ & $1^{+15}_{-1}$ & 57644.464507488(7) & $0.4^{+0.4}_{-0.3}$ & $0.7^{+0.6}_{-0.3}$ & $565^{+4}_{-2}$\\
B48.2$\dagger$ & $0^{+1300}_{-500}$ & $500^{+500}_{-400}$ & $0.7^{+26.2}_{-0.6}$ & 57644.4645075(2) & $0.9^{+3.2}_{-0.6}$ & $0.7^{+3.6}_{-0.4}$ & $600^{+100}_{-200}$\\
B49.1 & $1660^{+10}_{-10}$ & $140^{+20}_{-10}$ & $0.49^{+0.03}_{-0.03}$ & 57644.46475893(1) & $8.3^{+0.5}_{-0.5}$ & $2.0^{+0.7}_{-0.6}$ & $568^{+4}_{-4}$\\
B49.2 & $2400^{+700}_{-1400}$ & $2000^{+1000}_{-1000}$ & $0.16^{+0.05}_{-0.04}$ & 57644.464759903(1) & $0.2^{+0.1}_{-0.1}$ & $0.6^{+0.2}_{-0.1}$ & $561.3^{+0.3}_{-0.2}$\\
B50 & $1460^{+10}_{-10}$ & $90^{+10}_{-10}$ & $0.13^{+0.02}_{-0.01}$ & 57644.46476275(1) & $1.3^{+1.0}_{-0.9}$ & $1.7^{+0.6}_{-0.8}$ & $561^{+2}_{-2}$\\
B51$\dagger$ & $2500^{+600}_{-900}$ & $1000^{+1000}_{-700}$ & $0.3^{+0.2}_{-0.2}$ & 57644.465729923(7) & $1.4^{+0.6}_{-0.4}$ & $1.2^{+0.5}_{-0.4}$ & $569^{+1}_{-1}$\\
B52 & $1667^{+5}_{-4}$ & $73^{+6}_{-5}$ & $0.185^{+0.009}_{-0.009}$ & 57644.466222289(4) & $1.4^{+0.1}_{-0.2}$ & $0.6^{+0.2}_{-0.2}$ & $570^{+1}_{-1}$\\
B53 & $1720^{+30}_{-20}$ & $120^{+30}_{-20}$ & $0.19^{+0.03}_{-0.02}$ & 57644.468095365(4) & $1.5^{+0.2}_{-0.2}$ & $1.1^{+0.3}_{-0.3}$ & $572^{+1}_{-1}$\\
B54$*$ & $1600^{+600}_{-600}$ & $100^{+100}_{-100}$ & $0.0^{+0.1}_{-0.1}$ & 57644.47117767(7) & $0^{+10}_{-10}$ & $0.9^{+0.2}_{-0.2}$ & $560^{+40}_{-40}$\\
B55 & $1650^{+10}_{-10}$ & $100^{+10}_{-10}$ & $0.13^{+0.01}_{-0.01}$ & 57644.474717918(6) & $1.4^{+0.3}_{-0.2}$ & $1.3^{+0.5}_{-0.5}$ & $570^{+2}_{-2}$\\
B56 & $1706^{+4}_{-4}$ & $54^{+6}_{-5}$ & $0.16^{+0.01}_{-0.01}$ & 57644.477082041(3) & $0.9^{+0.2}_{-0.1}$ & $0.9^{+0.2}_{-0.2}$ & $560^{+2}_{-2}$\\
B57 & $1530^{+6}_{-6}$ & $186^{+6}_{-6}$ & $0.254^{+0.006}_{-0.005}$ & 57645.4110889611(4) & $0.48^{+0.03}_{-0.02}$ & $0.21^{+0.02}_{-0.02}$ & $561.75^{+0.06}_{-0.06}$\\
B58 & $1462^{+6}_{-6}$ & $78^{+6}_{-5}$ & $0.129^{+0.008}_{-0.008}$ & 57645.411651653(4) & $0.9^{+0.1}_{-0.1}$ & $0.4^{+0.1}_{-0.1}$ & $564.4^{+0.6}_{-0.7}$\\
B59 & $1537^{+5}_{-4}$ & $68^{+4}_{-4}$ & $0.2^{+0.01}_{-0.01}$ & 57645.411889086(9) & $2.2^{+0.4}_{-0.3}$ & $1.1^{+0.3}_{-0.3}$ & $568^{+2}_{-2}$\\
B60.1 & $3000^{+300}_{-1000}$ & $440^{+80}_{-220}$ & $4^{+6}_{-4}$ & 57645.412281872(4) & $0.8^{+0.2}_{-0.1}$ & $0.3^{+0.3}_{-0.2}$ & $566^{+2}_{-2}$\\
B60.2 & $2300^{+900}_{-600}$ & $500^{+300}_{-300}$ & $0.4^{+1.6}_{-0.2}$ & 57645.412281990(6) & $0.9^{+0.6}_{-0.5}$ & $2.5^{+0.6}_{-0.5}$ & $561^{+2}_{-2}$\\
B61$\dagger$ & $1000^{+1000}_{-1000}$ & $2800^{+900}_{-1100}$ & $0.25^{+0.08}_{-0.07}$ & 57645.41286869(2) & $2.0^{+2.0}_{-1.0}$ & $2^{+2}_{-1}$ & $580^{+3}_{-13}$\\
B62 & $1570^{+10}_{-10}$ & $110^{+10}_{-10}$ & $0.12^{+0.01}_{-0.009}$ & 57645.413644740(5) & $1.3^{+0.2}_{-0.2}$ & $0.6^{+0.3}_{-0.2}$ & $567^{+1}_{-1}$\\
B63 & $1280^{+10}_{-10}$ & $86^{+11}_{-9}$ & $0.1^{+0.01}_{-0.01}$ & 57645.41609534(1) & $0.8^{+0.2}_{-0.2}$ & $0.6^{+0.2}_{-0.1}$ & $562.0^{+0.8}_{-0.9}$\\
B64$\dagger$ & $2000^{+1000}_{-1000}$ & $3000^{+1000}_{-1000}$ & $0.32^{+0.09}_{-0.09}$ & 57645.41639521(1) & $1.4^{+0.5}_{-0.5}$ & $3^{+1}_{-1}$ & $564^{+3}_{-2}$\\
B65 & $1550^{+10}_{-10}$ & $110^{+20}_{-10}$ & $0.091^{+0.009}_{-0.009}$ & 57645.416564818(6) & $1.2^{+0.2}_{-0.2}$ & $0.6^{+0.3}_{-0.2}$ & $566.0^{+1.0}_{-1.0}$\\
B66 & $1440^{+10}_{-10}$ & $120^{+10}_{-10}$ & $0.105^{+0.009}_{-0.008}$ & 57645.417467306(6) & $1.6^{+0.2}_{-0.2}$ & - & $567.7^{+0.7}_{-0.7}$\\
B67 & $1640^{+30}_{-20}$ & $180^{+30}_{-30}$ & $0.099^{+0.009}_{-0.008}$ & 57645.417897463(2) & $0.8^{+0.1}_{-0.1}$ & $0.3^{+0.1}_{-0.1}$ & $564.8^{+0.5}_{-0.5}$\\
B68$\dagger$ & $2000^{+1000}_{-1000}$ & $2000^{+1000}_{-1000}$ & $0.2^{+0.05}_{-0.06}$ & 57645.419005902(8) & $1.0^{+0.6}_{-0.5}$ & $0.9^{+0.4}_{-0.4}$ & $567.9^{+0.9}_{-1.3}$\\
B69 & $1450^{+20}_{-10}$ & $80^{+10}_{-10}$ & $0.059^{+0.009}_{-0.009}$ & 57645.41920745(1) & $0.7^{+0.3}_{-0.3}$ & $0.5^{+0.3}_{-0.2}$ & $564^{+1}_{-1}$\\
B70$\dagger$ & $3100^{+200}_{-500}$ & $600^{+100}_{-100}$ & $0.9^{+1.7}_{-0.6}$ & 57645.419896226(4) & $0.8^{+0.3}_{-0.3}$ & $0.8^{+0.4}_{-0.3}$ & $564^{+1}_{-1}$\\
B71 & $1378^{+5}_{-4}$ & $78^{+5}_{-4}$ & $0.34^{+0.02}_{-0.02}$ & 57645.420265931(9) & $1.0^{+0.2}_{-0.2}$ & $2.6^{+0.2}_{-0.2}$ & $561.1^{+0.9}_{-1.0}$\\
B72$\dagger$ & $3100^{+200}_{-500}$ & $700^{+200}_{-100}$ & $1.2^{+3.4}_{-0.8}$ & 57645.420600439(9) & $1.2^{+0.7}_{-0.8}$ & $2^{+1}_{-1}$ & $559^{+2}_{-2}$\\
B73$\dagger$ & $3100^{+200}_{-500}$ & $600^{+100}_{-100}$ & $2^{+3}_{-1}$ & 57645.420679524(7) & $1.5^{+0.6}_{-0.8}$ & $1.7^{+0.8}_{-0.7}$ & $575^{+3}_{-3}$\\
B74$\dagger$ & $3100^{+200}_{-400}$ & $520^{+100}_{-90}$ & $5^{+12}_{-4}$ & 57645.420752363(6) & $1.2^{+0.8}_{-0.6}$ & $1.9^{+0.7}_{-0.9}$ & $551^{+11}_{-2}$\\
B75$\dagger$ & $2200^{+800}_{-1400}$ & $2700^{+900}_{-1200}$ & $0.39^{+0.07}_{-0.08}$ & 57645.421284056(4) & $0.9^{+0.3}_{-0.3}$ & $1.8^{+0.3}_{-0.3}$ & $567.6^{+0.9}_{-0.7}$\\
B76 & $1410^{+10}_{-350}$ & $90^{+20}_{-10}$ & $0.05^{+0.111}_{-0.006}$ & 57645.421290699(5) & $0.42^{+0.25}_{-0.09}$ & $0.14^{+0.42}_{-0.05}$ & $561.6^{+0.6}_{-0.5}$\\
B77 & $1312^{+5}_{-5}$ & $51^{+6}_{-6}$ & $0.12^{+0.01}_{-0.01}$ & 57645.42161300(2) & $1.3^{+0.5}_{-0.5}$ & $0.7^{+0.2}_{-0.2}$ & $566^{+2}_{-2}$\\
B78 & $1170^{+20}_{-40}$ & $80^{+40}_{-10}$ & $0.11^{+0.03}_{-0.02}$ & 57645.42184846(1) & $0.9^{+0.3}_{-0.2}$ & $0.28^{+0.14}_{-0.08}$ & $562.4^{+0.7}_{-0.9}$\\
B79 & $1702^{+4}_{-4}$ & $57^{+6}_{-5}$ & $0.18^{+0.01}_{-0.01}$ & 57645.421872443(3) & $1.2^{+0.2}_{-0.2}$ & $1.7^{+0.3}_{-0.3}$ & $568^{+2}_{-2}$\\
B80 & $1601^{+7}_{-8}$ & $81^{+8}_{-7}$ & $0.13^{+0.01}_{-0.01}$ & 57645.422454976(3) & $0.5^{+0.3}_{-0.2}$ & $1.3^{+0.2}_{-0.3}$ & $564.4^{+1.0}_{-0.8}$\\
B81 & $1720^{+390}_{-10}$ & $60^{+310}_{-20}$ & $0.05^{+0.1}_{-0.01}$ & 57645.423009490(6) & $0.78^{+0.08}_{-0.18}$ & $0.6^{+0.1}_{-0.2}$ & $563^{+8}_{-5}$\\
B82$\dagger$ & $3100^{+200}_{-400}$ & $580^{+60}_{-70}$ & $4^{+4}_{-2}$ & 57645.424145870(2) & $1.3^{+0.1}_{-0.1}$ & - & $569.2^{+0.7}_{-0.7}$\\
B83$\dagger$ & $2400^{+700}_{-1300}$ & $2000^{+2000}_{-1000}$ & $0.15^{+0.07}_{-0.04}$ & 57645.424617988(6) & $0.7^{+0.3}_{-0.3}$ & $0.4^{+0.2}_{-0.2}$ & $564.7^{+0.7}_{-0.5}$\\
B84$\dagger$ & $3000^{+300}_{-700}$ & $600^{+100}_{-200}$ & $1^{+3}_{-1}$ & 57645.425478263(8) & $1.0^{+0.8}_{-0.6}$ & $1.7^{+0.9}_{-0.9}$ & $563^{+2}_{-3}$\\
B85$*$ & $1310^{+20}_{-20}$ & $130^{+20}_{-20}$ & $0.11^{+0.02}_{-0.02}$ & 57645.426746546(2) & $0.01^{+0.06}_{-0.06}$ & $2.0^{+0.4}_{-0.4}$ & $566.1^{+0.2}_{-0.2}$\\
B86 & $1550^{+10}_{-10}$ & $80^{+10}_{-10}$ & $0.067^{+0.009}_{-0.008}$ & 57645.426792398(7) & $0.6^{+0.4}_{-0.3}$ & $0.9^{+0.3}_{-0.3}$ & $563^{+1}_{-1}$\\
B87 & $1760^{+440}_{-50}$ & $190^{+200}_{-50}$ & $0.2^{+0.38}_{-0.03}$ & 57645.426922532(4) & $1.4^{+0.2}_{-0.2}$ & $0.9^{+0.3}_{-0.3}$ & $571.1^{+0.9}_{-0.9}$\\
B88.1 & $2000^{+1000}_{-1000}$ & $2000^{+1000}_{-2000}$ & $0.17^{+0.06}_{-0.06}$ & 57645.427338932(7) & $0.7^{+0.4}_{-0.3}$ & $1.0^{+0.7}_{-0.5}$ & $561^{+2}_{-4}$\\
B88.2 & $1460^{+20}_{-10}$ & $130^{+20}_{-20}$ & $0.11^{+0.01}_{-0.01}$ & 57645.427339178(9) & $2.4^{+0.4}_{-0.3}$ & - & $561^{+1}_{-2}$\\
B89 & $1479^{+8}_{-8}$ & $120^{+8}_{-7}$ & $0.18^{+0.01}_{-0.01}$ & 57645.428904793(6) & $2.4^{+0.2}_{-0.2}$ & - & $569.0^{+0.7}_{-0.8}$\\
B90 & $1420^{+40}_{-500}$ & $120^{+2790}_{-30}$ & $0.09^{+0.11}_{-0.02}$ & 57645.42990044(2) & $2.4^{+0.6}_{-0.6}$ & $0.8^{+0.6}_{-0.3}$ & $565^{+2}_{-2}$\\
B91 & $1476^{+9}_{-9}$ & $81^{+10}_{-8}$ & $0.12^{+0.01}_{-0.01}$ & 57645.43034452(2) & $3.1^{+0.4}_{-0.4}$ & - & $572^{+2}_{-2}$\\
B92 & $1721^{+4}_{-4}$ & $39^{+6}_{-4}$ & $0.17^{+0.02}_{-0.02}$ & 57645.43044763(1) & $2.6^{+0.8}_{-0.7}$ & $3^{+1}_{-1}$ & $580^{+10}_{-10}$\\
B93.1 & $1591^{+9}_{-9}$ & $106^{+10}_{-9}$ & $0.126^{+0.008}_{-0.008}$ & 57645.430622487(3) & $1.2^{+0.1}_{-0.2}$ & $0.4^{+0.2}_{-0.2}$ & $565.3^{+0.8}_{-0.9}$\\
B93.2 & $1620^{+10}_{-10}$ & $120^{+20}_{-20}$ & $0.13^{+0.01}_{-0.01}$ & 57645.430622591(7) & $1.7^{+0.3}_{-0.3}$ & $0.8^{+0.4}_{-0.3}$ & $564^{+2}_{-2}$\\
B94$\dagger$ & $3100^{+200}_{-600}$ & $500^{+60}_{-120}$ & $7^{+10}_{-6}$ & 57645.431306274(4) & $1.1^{+0.2}_{-0.2}$ & $0.6^{+0.4}_{-0.3}$ & $565^{+2}_{-4}$\\
B95 & $1693^{+11}_{-8}$ & $90^{+20}_{-10}$ & $0.095^{+0.007}_{-0.007}$ & 57645.431478373(2) & $0.69^{+0.08}_{-0.08}$ & $0.22^{+0.12}_{-0.08}$ & $563.5^{+0.6}_{-0.5}$\\
B96$\dagger$ & $2000^{+1000}_{-2000}$ & $2800^{+800}_{-1100}$ & $0.2^{+0.06}_{-0.05}$ & 57645.43254531(2) & $2.1^{+0.8}_{-0.9}$ & $0.9^{+0.6}_{-0.3}$ & $565^{+2}_{-1}$\\
B97$\dagger$ & $2900^{+400}_{-800}$ & $800^{+500}_{-200}$ & $0.3^{+0.4}_{-0.1}$ & 57645.433086695(3) & $0.6^{+0.4}_{-0.4}$ & $1.0^{+0.4}_{-0.4}$ & $562.4^{+0.9}_{-0.5}$\\
B98 & $1667^{+7}_{-7}$ & $67^{+8}_{-7}$ & $0.094^{+0.01}_{-0.009}$ & 57645.434330453(5) & $1.1^{+0.2}_{-0.2}$ & $0.7^{+0.3}_{-0.3}$ & $559^{+2}_{-2}$\\
B99$\dagger$ & $2000^{+1000}_{-2000}$ & $2800^{+800}_{-1100}$ & $0.13^{+0.03}_{-0.03}$ & 57645.440066847(4) & $0.8^{+0.2}_{-0.2}$ & $0.3^{+0.2}_{-0.1}$ & $565.8^{+0.4}_{-0.4}$\\
B100 & $1688^{+4}_{-4}$ & $62^{+5}_{-5}$ & $0.154^{+0.008}_{-0.007}$ & 57645.440814641(2) & $1.0^{+0.1}_{-0.1}$ & $0.5^{+0.2}_{-0.2}$ & $567.0^{+1.0}_{-1.0}$\\
B101$*$ & $1510^{+20}_{-20}$ & $130^{+20}_{-20}$ & $0.042^{+0.006}_{-0.006}$ & 57645.441999925(3) & $0.87^{+0.02}_{-0.02}$ & - & $568.6^{+0.4}_{-0.4}$\\
B102 & $2000^{+1200}_{-300}$ & $300^{+300}_{-200}$ & $0.2^{+2.7}_{-0.1}$ & 57645.442100164(8) & $2.1^{+0.4}_{-0.4}$ & $0.8^{+0.6}_{-0.4}$ & $564^{+2}_{-2}$\\
B103 & $1470^{+10}_{-10}$ & $90^{+10}_{-10}$ & $0.08^{+0.01}_{-0.01}$ & 57645.44263325(1) & $1.4^{+0.3}_{-0.3}$ & $0.6^{+0.5}_{-0.3}$ & $562^{+1}_{-1}$\\
B104$*$ & $1460^{+60}_{-60}$ & $90^{+20}_{-20}$ & $0.07^{+0.09}_{-0.09}$ & 57645.4427413(1) & $0^{+2}_{-2}$ & $2.1^{+0.5}_{-0.5}$ & $569^{+8}_{-8}$\\
B105 & $1670^{+10}_{-10}$ & $110^{+20}_{-20}$ & $0.095^{+0.008}_{-0.007}$ & 57645.444480955(2) & $0.51^{+0.1}_{-0.09}$ & $0.5^{+0.1}_{-0.1}$ & $565.4^{+0.5}_{-0.5}$\\
B106 & $1480^{+7}_{-8}$ & $97^{+10}_{-9}$ & $0.16^{+0.01}_{-0.01}$ & 57645.444919472(7) & $2.0^{+0.2}_{-0.2}$ & $0.5^{+0.2}_{-0.1}$ & $566^{+1}_{-1}$\\
B107 & $2800^{+300}_{-1000}$ & $370^{+70}_{-260}$ & $10^{+10}_{-10}$ & 57645.445443070(5) & $1.2^{+0.3}_{-0.3}$ & $0.9^{+0.4}_{-0.4}$ & $561^{+3}_{-2}$\\
B108 & $1488^{+4}_{-4}$ & $83^{+4}_{-4}$ & $0.141^{+0.006}_{-0.006}$ & 57645.448802883(2) & $0.66^{+0.03}_{-0.03}$ & - & $561.1^{+0.3}_{-0.3}$\\
B109 & $1460^{+5}_{-5}$ & $87^{+5}_{-5}$ & $0.24^{+0.01}_{-0.01}$ & 57645.449987035(8) & $2.8^{+0.2}_{-0.2}$ & - & $568^{+1}_{-1}$\\
B110$*$ & $1620^{+10}_{-10}$ & $100^{+10}_{-10}$ & $0.1^{+0.01}_{-0.01}$ & 57645.451201066(8) & $1.7^{+0.4}_{-0.4}$ & $1.3^{+0.5}_{-0.5}$ & $561^{+2}_{-2}$\\
B111 & $1469^{+6}_{-6}$ & $58^{+7}_{-6}$ & $0.109^{+0.01}_{-0.009}$ & 57645.45198993(1) & $1.6^{+0.2}_{-0.2}$ & $0.5^{+0.2}_{-0.1}$ & $563^{+2}_{-2}$\\
B112 & $1442^{+4}_{-5}$ & $68^{+4}_{-4}$ & $0.142^{+0.008}_{-0.008}$ & 57645.453426198(4) & $0.59^{+0.08}_{-0.07}$ & $0.4^{+0.07}_{-0.06}$ & $563.1^{+0.6}_{-0.6}$\\
B113 & $1699^{+4}_{-4}$ & $68^{+6}_{-5}$ & $0.29^{+0.01}_{-0.01}$ & 57645.453639067(4) & $2.5^{+0.1}_{-0.2}$ & $0.6^{+0.3}_{-0.2}$ & $569^{+2}_{-2}$\\
B114 & $1570^{+20}_{-20}$ & $110^{+20}_{-20}$ & $0.07^{+0.01}_{-0.01}$ & 57645.453640216(3) & $0.3^{+0.2}_{-0.1}$ & $1.4^{+0.3}_{-0.3}$ & $566.5^{+0.7}_{-0.8}$\\
B115 & $1730^{+30}_{-10}$ & $90^{+20}_{-20}$ & $0.19^{+0.03}_{-0.02}$ & 57645.454258102(7) & $2.3^{+0.3}_{-0.3}$ & $0.9^{+0.6}_{-0.4}$ & $569^{+3}_{-3}$\\
B116$*$ & $1480^{+40}_{-40}$ & $260^{+60}_{-60}$ & $0.08^{+0.02}_{-0.02}$ & 57645.4544929400(9) & $0.05^{+0.07}_{-0.07}$ & $1.4^{+0.3}_{-0.3}$ & $565.7^{+0.2}_{-0.2}$\\
B117 & $1580^{+20}_{-20}$ & $130^{+30}_{-20}$ & $0.1^{+0.02}_{-0.01}$ & 57645.45736147(1) & $1.8^{+0.9}_{-0.8}$ & $1.8^{+0.8}_{-0.8}$ & $563^{+3}_{-3}$\\
B118 & $1580^{+30}_{-20}$ & $130^{+30}_{-20}$ & $0.1^{+0.02}_{-0.01}$ & 57645.45736147(1) & $1.7^{+0.9}_{-0.8}$ & $1.8^{+0.9}_{-0.8}$ & $563^{+3}_{-3}$\\
B119 & $1670^{+60}_{-20}$ & $170^{+60}_{-30}$ & $0.21^{+0.04}_{-0.02}$ & 57645.458536220(6) & $1.2^{+0.4}_{-0.3}$ & $2.6^{+0.5}_{-0.5}$ & $569^{+2}_{-2}$\\
B120 & $1690^{+1040}_{-30}$ & $130^{+380}_{-30}$ & $0.09^{+0.87}_{-0.01}$ & 57645.459103357(6) & $0.8^{+0.3}_{-0.5}$ & $1.2^{+0.5}_{-0.4}$ & $566^{+2}_{-2}$\\
B121.1 & $1612^{+2}_{-2}$ & $90^{+2}_{-2}$ & $0.394^{+0.007}_{-0.007}$ & 57645.460053270(1) & $0.82^{+0.04}_{-0.04}$ & $0.25^{+0.06}_{-0.07}$ & $562.1^{+0.2}_{-0.2}$\\
B121.2 & $1321^{+2}_{-3}$ & $178^{+2}_{-2}$ & $1.73^{+0.02}_{-0.02}$ & 57645.4600533283(4) & $0.95^{+0.02}_{-0.02}$ & $0.36^{+0.02}_{-0.01}$ & $561.98^{+0.03}_{-0.03}$\\
B121.3 & $1181^{+9}_{-11}$ & $93^{+9}_{-8}$ & $0.35^{+0.03}_{-0.02}$ & 57645.460053409(4) & $1.22^{+0.09}_{-0.07}$ & - & $561.6^{+0.2}_{-0.3}$\\
B122 & $1405^{+4}_{-4}$ & $71^{+5}_{-5}$ & $0.22^{+0.01}_{-0.01}$ & 57645.462106655(9) & $2.3^{+0.2}_{-0.2}$ & $0.5^{+0.2}_{-0.1}$ & $565^{+1}_{-1}$\\
B123$*$ & $1690^{+20}_{-20}$ & $90^{+20}_{-20}$ & $0.09^{+0.02}_{-0.02}$ & 57645.462556118(6) & $1.1^{+0.4}_{-0.4}$ & $2.0^{+0.6}_{-0.6}$ & $567^{+3}_{-3}$\\
B124 & $1560^{+10}_{-20}$ & $150^{+20}_{-20}$ & $0.094^{+0.008}_{-0.008}$ & 57645.464052738(3) & $1.0^{+0.2}_{-0.2}$ & $0.5^{+0.2}_{-0.2}$ & $565.3^{+0.5}_{-0.6}$\\
B125 & $1600^{+10}_{-10}$ & $140^{+20}_{-20}$ & $0.121^{+0.01}_{-0.009}$ & 57645.464188555(4) & $1.2^{+0.2}_{-0.2}$ & $0.7^{+0.2}_{-0.2}$ & $564.4^{+0.8}_{-0.8}$\\
B126 & $1600^{+1190}_{-60}$ & $230^{+2380}_{-90}$ & $0.07^{+0.13}_{-0.02}$ & 57645.464503855(6) & $0.9^{+0.4}_{-0.5}$ & $0.9^{+0.6}_{-0.4}$ & $567^{+2}_{-2}$\\
B127 & $2000^{+1000}_{-1000}$ & $2000^{+1000}_{-2000}$ & $0.19^{+0.06}_{-0.11}$ & 57645.465133243(7) & $0.8^{+0.4}_{-0.4}$ & $1.2^{+0.6}_{-0.5}$ & $566.0^{+1.9}_{-0.7}$\\
B128$\dagger$ & $1000^{+1000}_{-1000}$ & $2700^{+900}_{-1500}$ & $0.25^{+0.05}_{-0.09}$ & 57645.466100959(6) & $1.1^{+0.2}_{-0.2}$ & $0.9^{+0.3}_{-0.3}$ & $567.0^{+0.7}_{-0.9}$\\
B129 & $1710^{+1380}_{-20}$ & $90^{+450}_{-30}$ & $0.11^{+4.56}_{-0.02}$ & 57645.466379997(5) & $1.0^{+0.3}_{-0.3}$ & $1.3^{+0.4}_{-0.4}$ & $573^{+2}_{-3}$\\
B130$\dagger$ & $2000^{+1000}_{-1000}$ & $3000^{+1000}_{-1000}$ & $0.18^{+0.05}_{-0.05}$ & 57645.46833947(1) & $1.4^{+0.4}_{-0.4}$ & $0.6^{+0.4}_{-0.2}$ & $565.5^{+1.0}_{-0.8}$\\
B131 & $1460^{+10}_{-10}$ & $90^{+10}_{-10}$ & $0.08^{+0.01}_{-0.01}$ & 57645.47236212(1) & $1.1^{+0.4}_{-0.3}$ & $0.7^{+0.3}_{-0.3}$ & $564^{+1}_{-2}$\\
B132 & $1720^{+80}_{-20}$ & $100^{+70}_{-20}$ & $0.09^{+0.03}_{-0.01}$ & 57645.474138540(3) & $0.7^{+0.1}_{-0.1}$ & $0.4^{+0.2}_{-0.2}$ & $561^{+1}_{-1}$\\
B133 & $1740^{+180}_{-50}$ & $230^{+110}_{-40}$ & $0.22^{+0.1}_{-0.03}$ & 57645.474448229(4) & $1.7^{+0.2}_{-0.2}$ & $0.7^{+0.3}_{-0.3}$ & $570.6^{+0.7}_{-0.7}$\\
\enddata
\tablecomments{1$\sigma$ errors on the fits are shown on superscript and subscript of each value in the table. For $\mu_t$, the error on the last significant digit is shown in parenthesis.}
\tablenotetext{a}{Burst IDs are chronological. Individual component number (N) for multi-component bursts are appended to the burst IDs. Bursts modeled only using \texttt{curve\_fit} are marked with $*$. Note that the errors on these bursts could be unreliable and may be either under or over-estimated}. Bursts that extend beyond the observable bandwidth can also have unreliable estimates of spectra parameters and fluence (see Section~\ref{sec:fitcaveats}). We mark those bursts with $\dagger$ to indicate that their fluence and spectra parameters could be unconstrained. 
\tablenotetext{b}{$\mu_t$ is the mean of the pulse profile in units of MJD. This can be considered as the arrival time of the pulse. It is referenced to the solar system barycenter, after correcting to infinite frequency using a DM of 560.5\dmunits.}
\tablenotetext{c}{$\tau$ is referred to 1~GHz.}
\end{deluxetable*}


==> Dense Sample of FRB121102 bursts/todo.tex <==
1. Introduction [KA, DA]
2. Data [KA, DA]
3. Methods 
4. Results
    - Burst Sample
        - Rerun Heimdall + Fetch [DA] 
            - Refer them to infinite freq, barycenter 
        - Get Burst TOAs [KA] https://iopscience.iop.org/article/10.3847/1538-4357/aaf6ef/pdf 
        - Calculate burst widths? [KA]
            - Simple widths reported by Heimdall OR
            - Fit the bursts with a template??? [optional] [KA]
        - Estimate burst flux [KA]
        - Estimate burst fluence [KA] 
        - Calculate Energy and luminosity of bursts []
    - Make burst energy distribution [Reshma]
        - estimate completeness, filter bursts above completeness
        - estimate gamma
    - DM analysis [optional] [KA]
        - str optimisind DM: https://github.com/danielemichilli/DM\_phase
        - Some discussion of sad trombone, sub burst drift rate, etc 
        
5. Discussion
    - Spectra 
        - Extract spectra of bursts
        - Fit spectra with a model (gaussian + a slope?) [optional]
    - Wait time [Evan] -- can use
        /hyrule/data/users/dagarwal/KG\_FRB121102/121102\_bursts.csv for now 
        - Use burst TOAs, get wait times
        - make wait time distribution
        - fit the distribution with something
    - Period search [Maura, Evan can help] -- can use
    /hyrule/data/users/dagarwal/KG\_FRB121102/121102\_bursts.csv for now 
        - Use techniques typically used for RRAT period searches
        - use frbpa
        - https://github.com/KshitijAggarwal/frbpa 
        - other methods?
        - https://github.com/evanocathain/Useful\_RRAT\_stuff/blob/master/getper.py 
    - burst rate? [Evan]
        - some discussion about this
        - Poisson vs Weibull: 
            - https://github.com/RuiLuoAstro/BayesWeib 
            - https://github.com/MJastro95/weibull\_analysis 
    - Progenitor models
        - need to do a quick literature review on FRB121102 theories
6. Conclusions

Tables:
1. Table with all burst properties: MJD, Width, Fluence, Freq bandwidth(?), DM

Figures: 
1. All Burst spectograms
2. Energy dist" 
3. Spectra (Update from fig 3 of Gourdji et al, to include actual burst spectras instead of just colored bands)
4. Wait time dist", with published points on it 
5. Peak of wait time dist" vs minimum energy burst used. Li et al says the wait time for all bursts is 70s while that of high energy bursts was 200. Maybe we can see something similar from this? 


Other: 
1. Maura to email Editor of APJ Letters to ask about page limits, etc 
2. DA to email all the authors of Gourdji et al 2019 and offering them to opt-in as co-authors.  

Relevant Links: 
https://ui.adsabs.harvard.edu/abs/2019ApJ...877L..19G/abstract
https://ui.adsabs.harvard.edu/abs/2021MNRAS.500..448C/abstract
https://arxiv.org/abs/2012.07303


Meeting: 
17 December: 
    1. Wait time: which log normal did they use, don't use the very small spacing bursts, mention the function in the paper, 
    2. Period: sim code by Maura, period diff code, Evan to try other techniques 
    3. Energy distribution: comparison with other papers. 
    4. Burst rate: only use bursts above completeness 
    5. nanograv does spectra temporal analysis code 

==> burst_table.tex <==
\startlongtable
\begin{deluxetable*}{lrrrrrrrrrrrrrrrrrrrrrr}
% \tablenum{1}
% \tablecaption{Astrometric Comparison \label{tab:astrometry}}
% \tablewidth{\linewidth}
\longrotatetable
% \tablehead{
% \colhead{Sr. No} & \multicolumn{2}{c}{Radio (J2000)} & \multicolumn{2}{c}{Optical (J2000)} & \multicolumn{2}{c}{Offset ($\arcsec$)}\\
% \colhead{} & \colhead{RA} & \colhead{DEC} & \colhead{RA} & \colhead{DEC} & \colhead{RA} & \colhead{DEC}}
\startdata
% \begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
% \rotatetable
% \toprule
% {} &  \$\textbackslash mu\_f\$ (MHz) &  upper error\$\textbackslash mu\_f\$ (MHz) &  lower error\$\textbackslash mu\_f\$ (MHz) &  \$\textbackslash sigma\_f\$ (MHz) &  upper error\$\textbackslash sigma\_f\$ (MHz) &  lower error\$\textbackslash sigma\_f\$ (MHz) &  \$S\$ (Jy ms) &  upper error\$S\$ (Jy ms) &  lower error\$S\$ (Jy ms) &  \$\textbackslash mu\_t\$ (ms) &  upper error\$\textbackslash mu\_t\$ (ms) &  lower error\$\textbackslash mu\_t\$ (ms) &  \$\textbackslash sigma\_t\$ (ms) &  upper error\$\textbackslash sigma\_t\$ (ms) &  lower error\$\textbackslash sigma\_t\$ (ms) &  \$\textbackslash tau\$ (ms) &  upper error\$\textbackslash tau\$ (ms) &  lower error\$\textbackslash tau\$ (ms) &  DM (pc cm\$\textasciicircum \{-3\}\$) &  upper errorDM (pc cm\$\textasciicircum \{-3\}\$) &  lower errorDM (pc cm\$\textasciicircum \{-3\}\$) &  comp\_num \\
% \midrule
0   &    3074.866031 &              2.235324e+02 &              5.558695e+02 &        549.818353 &                    83.033079 &                   111.124293 &     2.106578 &                3.684532 &                1.606049 &  57644.410073 &             3.601599e-09 &             4.030881e-09 &         1.066126 &                1.981733e-01 &                1.837101e-01 &     0.306613 &                0.169090 &                0.107359 &         563.878367 &                  1.017721e+00 &                  1.145842e+00 &         1 \\
1   &    2100.643913 &              9.380480e+02 &              1.617787e+03 &       2703.687541 &                   929.441672 &                  1238.095536 &     0.191984 &                0.048706 &                0.043850 &  57644.410158 &             4.198228e-09 &             4.241883e-09 &         0.661879 &                3.060655e-01 &                2.605480e-01 &     1.017467 &                0.422653 &                0.336476 &         562.082164 &                  7.254827e-01 &                  5.641742e-01 &         1 \\
2   &    3043.016847 &              2.468530e+02 &              5.551768e+02 &        651.601141 &                   126.841656 &                   138.216471 &     1.094175 &                1.498200 &                0.706197 &  57644.414124 &             4.416506e-09 &             3.798050e-09 &         1.002067 &                2.568850e-01 &                2.624549e-01 &     0.788696 &                0.357439 &                0.327918 &         567.458069 &                  9.422403e-01 &                  7.289469e-01 &         1 \\
3   &    1625.910301 &              1.097377e+01 &              1.112842e+01 &         81.941052 &                     8.484747 &                     7.630736 &     0.096903 &                0.010891 &                0.010307 &  57644.414475 &             7.814378e-09 &             7.028575e-09 &         1.441726 &                2.798057e-01 &                3.051317e-01 &     0.517916 &                0.289825 &                0.204750 &         562.070297 &                  2.744559e+00 &                  3.221510e+00 &         1 \\
4   &    1554.209322 &              1.074664e+01 &              1.097490e+01 &         96.109806 &                    12.949014 &                    10.630297 &     0.074124 &                0.007772 &                0.007439 &  57644.414879 &             4.285539e-09 &             4.634785e-09 &         0.846018 &                1.630260e-01 &                1.652373e-01 &     0.290967 &                0.183909 &                0.113241 &         560.324649 &                  9.282696e-01 &                  9.499163e-01 &         1 \\
5   &    3050.184527 &              2.119497e+02 &              2.986416e+02 &        450.459497 &                    63.929215 &                    76.973965 &    18.396136 &               16.474113 &               12.489799 &  57644.415378 &             9.298674e-09 &             1.039007e-08 &         1.931171 &                4.773695e-01 &                5.216117e-01 &     1.503911 &                1.301241 &                0.813175 &         568.583506 &                  3.498099e+00 &                  4.353664e+00 &         1 \\
6   &    1691.877912 &              1.267490e+01 &              9.384032e+00 &         88.653272 &                    15.908305 &                    11.837436 &     0.138823 &                0.011258 &                0.009906 &  57644.416315 &             4.503818e-09 &             4.867616e-09 &         1.487408 &                1.787762e-01 &                2.148986e-01 &     0.576520 &                0.318885 &                0.242019 &         571.851847 &                  1.470420e+00 &                  1.375934e+00 &         1 \\
7   &    1264.593451 &              1.026780e+01 &              9.957336e+00 &         67.355321 &                     8.601894 &                     7.840279 &     0.134822 &                0.020072 &                0.018831 &  57644.418307 &             6.829941e-08 &             8.276402e-08 &         2.951750 &                1.149607e+00 &                1.022370e+00 &     1.572956 &                0.599972 &                0.503402 &         562.018317 &                  5.858997e+00 &                  4.594390e+00 &         1 \\
8   &    3060.064914 &              2.280279e+02 &              5.946436e+02 &        510.421523 &                    64.135840 &                   111.276660 &     5.938947 &                9.144948 &                4.880618 &  57644.420509 &             4.096364e-09 &             4.336471e-09 &         1.189536 &                2.167979e-01 &                2.476828e-01 &     0.515828 &                0.287973 &                0.221253 &         570.290783 &                  1.691348e+00 &                  1.591659e+00 &         1 \\
9   &    2023.841501 &              9.894923e+02 &              1.662523e+03 &       2586.118211 &                  1009.910387 &                  1374.250034 &     0.151061 &                0.052290 &                0.041881 &  57644.421105 &             1.192529e-08 &             1.271837e-08 &         1.515181 &                5.527047e-01 &                5.232992e-01 &     0.739936 &                0.956501 &                0.352010 &         570.114031 &                  1.427338e+00 &                  1.930761e+00 &         1 \\
10  &    2855.697638 &              3.896675e+02 &              1.029775e+03 &       1048.190129 &                  1990.096884 &                   381.871492 &     0.233454 &                0.473724 &                0.079166 &  57644.427377 &             4.161848e-09 &             4.431058e-09 &         0.665876 &                2.837010e-01 &                3.299061e-01 &     0.591814 &                0.499724 &                0.308283 &         565.578180 &                  7.605473e-01 &                  5.649291e-01 &         1 \\
11  &    3103.820597 &              2.018182e+02 &              4.271795e+02 &        600.939265 &                   128.391839 &                   107.392819 &     2.734857 &                6.614627 &                1.852813 &  57644.427940 &             1.626177e-08 &             1.920125e-08 &         4.157687 &                8.739811e-01 &                9.919716e-01 &     1.820251 &                1.663655 &                0.835002 &         576.108744 &                  4.475180e+00 &                  5.135311e+00 &         1 \\
12  &    2991.434179 &              2.896015e+02 &              7.154517e+02 &        655.332362 &                   124.101717 &                   183.316387 &     1.338308 &                1.723632 &                0.936200 &  57644.428594 &             8.505594e-09 &             7.770723e-09 &         1.907938 &                4.269817e-01 &                4.178503e-01 &     1.526522 &                0.633527 &                0.631164 &         567.646156 &                  2.254513e+00 &                  2.149866e+00 &         1 \\
13  &    1698.759487 &              1.366499e+01 &              9.111177e+00 &         74.723176 &                    15.406403 &                     9.972977 &     0.089443 &                0.008710 &                0.007885 &  57644.430170 &             2.240995e-09 &             2.284651e-09 &         0.687118 &                1.052845e-01 &                1.099720e-01 &     0.332783 &                0.167763 &                0.144788 &         568.703039 &                  9.671064e-01 &                  9.771692e-01 &         1 \\
14  &    1753.113555 &              1.375950e+03 &              7.232516e+01 &        201.834574 &                   389.647488 &                    59.315807 &     0.161804 &                3.671485 &                0.031272 &  57644.430171 &             4.030881e-09 &             3.943569e-09 &         1.383852 &                1.743766e-01 &                1.975387e-01 &     0.661673 &                0.274440 &                0.258215 &         568.004469 &                  1.179303e+00 &                  1.158146e+00 &         1 \\
15  &    1469.638266 &              1.206921e+01 &              1.418449e+01 &        110.168894 &                    15.648925 &                    12.536650 &     0.096237 &                0.008865 &                0.008593 &  57644.431295 &             4.285539e-09 &             4.605681e-09 &         0.825079 &                1.765630e-01 &                1.691157e-01 &     0.489867 &                0.166650 &                0.169472 &         565.606060 &                  6.900090e-01 &                  6.774787e-01 &         1 \\
16  &    1344.471659 &              7.231304e+01 &              1.397881e+03 &       1123.000215 &                  2074.461619 &                   999.931723 &     0.172616 &                0.108263 &                0.085568 &  57644.432235 &             2.412708e-08 &             1.642184e-08 &         2.041703 &                9.811888e-01 &                6.821793e-01 &     1.074649 &                0.518550 &                0.405960 &         569.606721 &                  1.532792e+00 &                  2.172629e+00 &         1 \\
17  &    1753.873529 &              3.883385e+01 &              1.888832e+01 &         96.044583 &                    23.238518 &                    13.841937 &     0.136800 &                0.031607 &                0.015147 &  57644.432243 &             1.062290e-09 &             1.200533e-09 &         0.590009 &                4.580417e-02 &                4.600942e-02 &     0.157519 &                0.085570 &                0.052893 &         561.341086 &                  5.100551e-01 &                  5.005275e-01 &         1 \\
18  &    1682.086671 &              1.440497e+03 &              3.403930e+01 &        126.720043 &                   482.469828 &                    36.524709 &     0.062906 &                1.502574 &                0.013961 &  57644.434045 &             3.630703e-09 &             3.819878e-09 &         0.649565 &                1.837050e-01 &                1.652012e-01 &     0.415542 &                0.434776 &                0.227983 &         561.944971 &                  1.251747e+00 &                  3.338278e+00 &         1 \\
19  &    1438.436789 &              1.209237e+01 &              1.271892e+01 &         96.874532 &                    15.153189 &                    12.912619 &     0.120952 &                0.013904 &                0.013317 &  57644.436366 &             1.943408e-08 &             1.943408e-08 &         2.114945 &                5.862555e-01 &                5.351130e-01 &     1.171342 &                0.484130 &                0.424576 &         568.292911 &                  2.401008e+00 &                  2.515646e+00 &         1 \\
20  &    1501.654308 &              6.318258e+00 &              6.421393e+00 &        100.308781 &                     8.131903 &                     7.255264 &     0.191268 &                0.010069 &                0.009738 &  57644.438795 &             4.292815e-09 &             4.314643e-09 &         1.569189 &                1.411267e-01 &                1.505217e-01 &     0.466902 &                0.136887 &                0.131183 &         566.614957 &                  7.196468e-01 &                  7.352750e-01 &         1 \\
21  &    1410.170642 &              7.569828e+00 &              7.570620e+00 &         78.703681 &                     8.584276 &                     7.667938 &     0.136800 &                0.012764 &                0.011952 &  57644.438845 &             1.407898e-08 &             1.453009e-08 &         1.712679 &                2.874023e-01 &                3.804301e-01 &     0.645991 &                0.371919 &                0.266140 &         564.208575 &                  1.407150e+00 &                  1.391008e+00 &         1 \\
22  &    1476.816576 &              1.764255e+01 &              1.837630e+01 &        122.879736 &                    20.312368 &                    16.493155 &     0.077668 &                0.012491 &                0.010282 &  57644.439213 &             8.963980e-09 &             7.494236e-09 &         1.181245 &                3.026901e-01 &                3.555885e-01 &     0.593462 &                0.562631 &                0.291490 &         562.531953 &                  9.726264e-01 &                  1.335052e+00 &         1 \\
23  &    2559.531270 &              6.121318e+02 &              1.391842e+03 &       2052.859562 &                  1413.031171 &                  1089.324504 &     0.271982 &                0.101074 &                0.063633 &  57644.440689 &             5.151378e-09 &             5.631591e-09 &         1.276658 &                4.331835e-01 &                3.749133e-01 &     1.007187 &                0.405653 &                0.335115 &         567.032343 &                  8.125252e-01 &                  9.055199e-01 &         1 \\
24  &    1706.895880 &              5.255398e+00 &              4.676408e+00 &         60.556705 &                     5.794844 &                     4.920802 &     0.235009 &                0.012553 &                0.012401 &  57644.442998 &             5.384209e-09 &             5.777110e-09 &         2.754589 &                1.939485e-01 &                2.101955e-01 &     0.724094 &                0.360728 &                0.236483 &         575.259473 &                  2.618152e+00 &                  2.674777e+00 &         1 \\
25  &    3103.200327 &              1.946750e+02 &              4.059270e+02 &        474.923047 &                    65.301911 &                    88.311098 &    13.562077 &               23.919749 &               10.923801 &  57644.443589 &             1.658918e-08 &             2.646266e-08 &         2.964734 &                1.617569e+00 &                1.275405e+00 &     2.282858 &                1.555881 &                1.228661 &         574.414294 &                  1.111077e+01 &                  6.138218e+00 &         1 \\
26  &    1411.850547 &              2.385258e+01 &              1.689906e+01 &        133.180398 &                    28.234492 &                    15.536819 &     0.065361 &                0.006609 &                0.008498 &  57644.443590 &             3.012246e-09 &             3.965397e-09 &         0.582531 &                1.138658e-01 &                8.714409e-02 &     0.143780 &                0.100254 &                0.041402 &         562.804360 &                  4.703068e-01 &                  3.794158e-01 &         1 \\
27  &    1618.330258 &              1.839669e+01 &              1.603617e+01 &        110.114902 &                    20.796256 &                    15.157108 &     0.098552 &                0.014725 &                0.013936 &  57644.445225 &             8.025381e-09 &             6.562914e-09 &         0.908927 &                5.076986e-01 &                4.568527e-01 &     1.941624 &                0.717931 &                0.933281 &         567.429180 &                  1.547327e+00 &                  1.507595e+00 &         1 \\
28  &    1503.320019 &              1.389504e+01 &              1.780477e+01 &        126.004337 &                    12.821785 &                    12.278029 &     0.056761 &                0.009834 &                0.005824 &  57644.446788 &             1.025910e-09 &             1.738954e-09 &         0.210515 &                4.084608e-02 &                4.368951e-02 &     0.117640 &                0.130097 &                0.050336 &         560.903446 &                  1.483747e-01 &                  1.509667e-01 &         1 \\
29  &    1588.192968 &              1.037492e+01 &              1.034613e+01 &         81.401848 &                    10.775125 &                     9.141235 &     0.117638 &                0.017005 &                0.015048 &  57644.447568 &             8.825737e-09 &             7.421477e-09 &         1.132266 &                4.550410e-01 &                3.937062e-01 &     2.031254 &                0.766859 &                0.658937 &         559.847303 &                  2.627435e+00 &                  2.679809e+00 &         1 \\
30  &    1668.190100 &              1.470283e+01 &              1.166082e+01 &        108.039238 &                    18.422603 &                    15.684084 &     0.098879 &                0.008575 &                0.007991 &  57644.449916 &             2.844899e-09 &             2.881279e-09 &         0.933206 &                1.603030e-01 &                2.302788e-01 &     0.385870 &                0.233127 &                0.162074 &         565.960796 &                  7.981315e-01 &                  7.370288e-01 &         1 \\
31  &    1682.778949 &              1.212718e+01 &              9.065245e+00 &        123.545326 &                    15.464187 &                    12.451648 &     0.220447 &                0.012752 &                0.011042 &  57644.451605 &             1.367880e-09 &             1.295120e-09 &         0.794652 &                9.527094e-02 &                8.914728e-02 &     0.861114 &                0.114901 &                0.116967 &         568.158109 &                  4.500589e-01 &                  4.575727e-01 &         1 \\
32  &    3133.007516 &              1.752323e+02 &              3.555619e+02 &        521.759457 &                    53.669815 &                    71.453022 &    10.750999 &               12.859349 &                7.172429 &  57644.452390 &             6.199116e-09 &             5.813490e-09 &         1.820845 &                3.211144e-01 &                3.441520e-01 &     1.062797 &                0.519755 &                0.450985 &         568.780888 &                  2.326107e+00 &                  3.967006e+00 &         1 \\
33  &    1706.506824 &              1.486371e+03 &              5.735066e+01 &        161.988513 &                   474.968514 &                    74.460338 &     0.073680 &                1.805807 &                0.017110 &  57644.453937 &             4.474714e-09 &             3.812602e-09 &         0.868842 &                1.955563e-01 &                4.358830e-01 &     0.464707 &                0.410655 &                0.224231 &         562.476867 &                  1.387534e+00 &                  1.204624e+00 &         1 \\
34  &    1371.004537 &              2.147831e+00 &              2.229256e+00 &         61.489048 &                     2.308837 &                     2.215078 &     0.413836 &                0.012679 &                0.012414 &  57644.454477 &             8.207280e-09 &             8.236384e-09 &         2.765609 &                1.714455e-01 &                2.043305e-01 &     0.579716 &                0.140395 &                0.113697 &         569.599056 &                  8.297861e-01 &                  8.262580e-01 &         1 \\
35  &     894.507502 &              7.620895e+02 &              1.126316e+03 &       2011.222953 &                  1426.993479 &                  1715.332126 &     0.147564 &                0.044851 &                0.085532 &  57644.457883 &             3.143214e-09 &             2.633897e-09 &         0.501936 &                1.164454e-01 &                1.082587e-01 &     0.230207 &                0.135557 &                0.089106 &         561.936050 &                  2.577489e-01 &                  2.205913e-01 &         1 \\
36  &    1459.305290 &              1.016497e+01 &              1.073324e+01 &         85.536712 &                    10.825652 &                     9.552485 &     0.131336 &                0.015209 &                0.013934 &  57644.464763 &             1.196167e-08 &             1.225999e-08 &         1.335409 &                1.016914e+00 &                8.644005e-01 &     1.724340 &                0.599098 &                0.805386 &         561.484822 &                  2.394596e+00 &                  2.044029e+00 &         1 \\
37  &    2510.246818 &              6.473744e+02 &              9.160298e+02 &        951.881154 &                  1033.817204 &                   662.665551 &     0.315935 &                0.218037 &                0.191947 &  57644.465730 &             5.908078e-09 &             7.137714e-09 &         1.415205 &                5.608766e-01 &                3.817702e-01 &     1.156707 &                0.460134 &                0.407823 &         568.521350 &                  1.155807e+00 &                  1.180769e+00 &         1 \\
38  &    1667.343509 &              4.503356e+00 &              4.432376e+00 &         73.207001 &                     5.716007 &                     5.032887 &     0.184765 &                0.008873 &                0.008831 &  57644.466222 &             3.579771e-09 &             3.499736e-09 &         1.433698 &                1.459874e-01 &                1.585554e-01 &     0.631623 &                0.244238 &                0.239255 &         569.802339 &                  1.053614e+00 &                  1.049471e+00 &         1 \\
39  &    1715.831245 &              3.339547e+01 &              1.762622e+01 &        121.070355 &                    28.866351 &                    20.328101 &     0.191454 &                0.025641 &                0.016973 &  57644.468095 &             3.943569e-09 &             3.587047e-09 &         1.465745 &                2.426216e-01 &                2.234313e-01 &     1.124791 &                0.307505 &                0.343491 &         571.848392 &                  1.392233e+00 &                  1.385351e+00 &         1 \\
40  &    1648.709455 &              1.238575e+01 &              1.047486e+01 &         95.229489 &                    12.159934 &                     9.821915 &     0.130790 &                0.013169 &                0.011964 &  57644.474718 &             5.573384e-09 &             5.427864e-09 &         1.406831 &                2.669049e-01 &                2.417088e-01 &     1.285286 &                0.485314 &                0.460723 &         569.847221 &                  1.555281e+00 &                  1.583119e+00 &         1 \\
41  &    1706.126003 &              4.455174e+00 &              4.011692e+00 &         53.672923 &                     6.001413 &                     4.867634 &     0.161523 &                0.010557 &                0.010259 &  57644.477082 &             2.946763e-09 &             2.612069e-09 &         0.884572 &                1.603169e-01 &                1.382247e-01 &     0.909979 &                0.215300 &                0.222388 &         559.703915 &                  1.616269e+00 &                  1.655394e+00 &         1 \\
42  &    1530.213173 &              5.727281e+00 &              5.661187e+00 &        185.967267 &                     6.268319 &                     6.118243 &     0.253702 &                0.005759 &                0.005462 &  57645.411089 &             4.074536e-10 &             4.074536e-10 &         0.480743 &                2.506085e-02 &                2.396012e-02 &     0.209457 &                0.023042 &                0.024457 &         561.746352 &                  6.052966e-02 &                  6.053392e-02 &         1 \\
43  &    1462.010835 &              5.553152e+00 &              5.594528e+00 &         77.625610 &                     5.829904 &                     5.415621 &     0.129210 &                0.008103 &                0.007884 &  57645.411652 &             4.329195e-09 &             4.220055e-09 &         0.938840 &                1.489901e-01 &                1.358012e-01 &     0.410036 &                0.113743 &                0.119876 &         564.370351 &                  6.195938e-01 &                  6.505681e-01 &         1 \\
44  &    1536.584557 &              4.637798e+00 &              4.457538e+00 &         68.150290 &                     4.482496 &                     4.085008 &     0.201344 &                0.012168 &                0.011755 &  57645.411889 &             9.044015e-09 &             9.080395e-09 &         2.206685 &                3.529253e-01 &                3.360156e-01 &     1.098157 &                0.315794 &                0.345030 &         567.830593 &                  2.087382e+00 &                  2.019221e+00 &         1 \\
45  &    1437.894307 &              1.344831e+03 &              1.433164e+03 &       2809.123585 &                   854.915279 &                  1136.821635 &     0.250711 &                0.080272 &                0.067918 &  57645.412869 &             1.891021e-08 &             1.730950e-08 &         1.942670 &                2.359892e+00 &                9.978470e-01 &     2.483146 &                1.716731 &                1.152991 &         579.730888 &                  2.814247e+00 &                  1.336684e+01 &         1 \\
46  &    1574.834447 &              1.051695e+01 &              1.102502e+01 &        110.151733 &                    14.569998 &                    11.252887 &     0.119899 &                0.009656 &                0.009066 &  57645.413645 &             4.591129e-09 &             4.598405e-09 &         1.308066 &                2.061113e-01 &                2.173937e-01 &     0.611663 &                0.268956 &                0.237248 &         567.219651 &                  1.148594e+00 &                  1.250406e+00 &         1 \\
47  &    1276.268654 &              9.907018e+00 &              1.046554e+01 &         85.622207 &                    10.744013 &                     8.672704 &     0.103104 &                0.011392 &                0.010585 &  57645.416095 &             1.221633e-08 &             1.124135e-08 &         0.772538 &                2.422718e-01 &                2.069768e-01 &     0.601874 &                0.152525 &                0.139996 &         562.017081 &                  7.870831e-01 &                  8.581060e-01 &         1 \\
48  &    1824.658692 &              1.127025e+03 &              1.414468e+03 &       2631.968332 &                   983.372832 &                  1385.619418 &     0.315998 &                0.086042 &                0.093915 &  57645.416395 &             1.063017e-08 &             1.590524e-08 &         1.354395 &                4.831073e-01 &                4.717508e-01 &     2.528038 &                1.184442 &                1.253809 &         564.386687 &                  2.763047e+00 &                  1.763732e+00 &         1 \\
49  &    1549.302740 &              1.238233e+01 &              1.253089e+01 &        108.165411 &                    16.051127 &                    13.199135 &     0.091439 &                0.009100 &                0.008511 &  57645.416565 &             6.133632e-09 &             5.755282e-09 &         1.190103 &                2.234641e-01 &                2.328542e-01 &     0.572738 &                0.286101 &                0.236289 &         565.703772 &                  9.632887e-01 &                  1.132814e+00 &         1 \\
50  &    1438.283092 &              1.156853e+01 &              1.209166e+01 &        117.724997 &                    12.750942 &                    11.357021 &     0.104655 &                0.008589 &                0.008352 &  57645.417467 &             6.140908e-09 &             6.002665e-09 &         1.597562 &                1.640428e-01 &                1.502190e-01 &          NaN &                     NaN &                     NaN &         567.670017 &                  7.432870e-01 &                  7.140798e-01 &         1 \\
51  &    1639.949905 &              2.627778e+01 &              1.879937e+01 &        175.242092 &                    34.953992 &                    27.143575 &     0.099303 &                0.008999 &                0.007899 &  57645.417897 &             1.913577e-09 &             1.942681e-09 &         0.823244 &                1.052152e-01 &                1.134531e-01 &     0.313503 &                0.148577 &                0.118934 &         564.754956 &                  4.700210e-01 &                  5.049791e-01 &         1 \\
52  &    2078.748339 &              9.504298e+02 &              1.288309e+03 &       2389.310168 &                  1165.979362 &                  1376.413304 &     0.196102 &                0.051064 &                0.060172 &  57645.419006 &             9.793439e-09 &             5.733455e-09 &         0.976380 &                5.603939e-01 &                4.866207e-01 &     0.887142 &                0.412448 &                0.356371 &         567.938667 &                  9.387700e-01 &                  1.321105e+00 &         1 \\
53  &    1452.437833 &              1.565797e+01 &              1.373409e+01 &         84.319910 &                    13.939876 &                    12.536747 &     0.059015 &                0.008613 &                0.009182 &  57645.419207 &             1.065928e-08 &             8.789357e-09 &         0.732501 &                3.128089e-01 &                3.145160e-01 &     0.523796 &                0.284610 &                0.220513 &         564.482479 &                  1.319433e+00 &                  1.346727e+00 &         1 \\
54  &    3084.578024 &              2.173158e+02 &              4.594366e+02 &        636.750129 &                   146.021669 &                   116.310538 &     0.897362 &                1.698278 &                0.574115 &  57645.419896 &             3.594323e-09 &             3.739842e-09 &         0.793183 &                3.371007e-01 &                2.877284e-01 &     0.752933 &                0.389404 &                0.331647 &         563.805103 &                  1.354127e+00 &                  1.352878e+00 &         1 \\
55  &    1377.852703 &              4.584987e+00 &              4.450188e+00 &         78.105911 &                     4.514130 &                     4.201103 &     0.343787 &                0.018127 &                0.018032 &  57645.420266 &             9.742507e-09 &             8.847564e-09 &         0.997937 &                2.319654e-01 &                2.114472e-01 &     2.576255 &                0.240224 &                0.222771 &         561.077047 &                  8.693652e-01 &                  9.538554e-01 &         1 \\
56  &    3083.245091 &              2.168906e+02 &              4.631372e+02 &        655.946966 &                   239.483604 &                   138.808615 &     1.153999 &                3.418312 &                0.797813 &  57645.420600 &             1.075387e-08 &             7.064955e-09 &         1.165608 &                6.735023e-01 &                8.338094e-01 &     2.089366 &                1.334955 &                1.169319 &         558.973786 &                  1.589612e+00 &                  2.256962e+00 &         1 \\
57  &    3080.006672 &              2.201802e+02 &              4.673256e+02 &        616.137403 &                   135.897106 &                   115.434427 &     1.510880 &                2.934927 &                1.008181 &  57645.420680 &             7.355993e-09 &             5.951733e-09 &         1.541820 &                6.136190e-01 &                7.856533e-01 &     1.658819 &                0.833653 &                0.740008 &         574.831291 &                  2.985381e+00 &                  2.848148e+00 &         1 \\
58  &    3134.262020 &              1.766043e+02 &              3.970975e+02 &        522.748261 &                    95.546504 &                    87.129776 &     4.741475 &               12.315336 &                3.561078 &  57645.420752 &             5.755282e-09 &             6.642949e-09 &         1.156756 &                8.351653e-01 &                6.014175e-01 &     1.862063 &                0.695683 &                0.873280 &         551.223922 &                  1.070645e+01 &                  2.455613e+00 &         1 \\
59  &    2192.334917 &              8.460233e+02 &              1.430771e+03 &       2710.988090 &                   921.007274 &                  1205.982722 &     0.391624 &                0.068889 &                0.079138 &  57645.421284 &             3.819878e-09 &             4.110916e-09 &         0.901937 &                3.400151e-01 &                2.823390e-01 &     1.814649 &                0.345687 &                0.318261 &         567.621215 &                  9.428158e-01 &                  6.959242e-01 &         1 \\
60  &    1408.568517 &              1.358635e+01 &              3.520050e+02 &         93.912852 &                    22.657394 &                    13.599363 &     0.049803 &                0.111454 &                0.005826 &  57645.421291 &             5.304173e-09 &             4.562025e-09 &         0.424682 &                2.453251e-01 &                8.717474e-02 &     0.140114 &                0.415216 &                0.054827 &         561.627252 &                  5.751793e-01 &                  4.948632e-01 &         1 \\
61  &    1311.987182 &              5.233456e+00 &              5.437590e+00 &         51.087297 &                     6.497108 &                     5.735694 &     0.122126 &                0.010987 &                0.011020 &  57645.421613 &             1.741137e-08 &             2.342858e-08 &         1.293325 &                4.651924e-01 &                5.225449e-01 &     0.692962 &                0.228425 &                0.215155 &         565.730861 &                  2.180546e+00 &                  1.593501e+00 &         1 \\
62  &    1172.297671 &              1.718399e+01 &              3.618796e+01 &         77.921133 &                    35.690074 &                    13.469704 &     0.108801 &                0.027883 &                0.015008 &  57645.421848 &             1.339504e-08 &             1.594890e-08 &         0.874872 &                2.837906e-01 &                2.435208e-01 &     0.282655 &                0.141733 &                0.081908 &         562.413441 &                  7.209325e-01 &                  8.760608e-01 &         1 \\
63  &    1702.012160 &              4.147355e+00 &              4.029573e+00 &         56.897315 &                     5.611201 &                     4.808106 &     0.176938 &                0.011188 &                0.010390 &  57645.421872 &             3.383320e-09 &             3.368768e-09 &         1.192419 &                2.046551e-01 &                1.782679e-01 &     1.686745 &                0.290801 &                0.296226 &         568.033427 &                  2.209772e+00 &                  2.176216e+00 &         1 \\
64  &    1600.554398 &              7.277823e+00 &              7.744704e+00 &         80.877312 &                     8.360896 &                     7.439249 &     0.128628 &                0.009511 &                0.009663 &  57645.422455 &             3.034074e-09 &             2.939487e-09 &         0.522650 &                2.880950e-01 &                1.816306e-01 &     1.317777 &                0.235973 &                0.273817 &         564.441465 &                  1.034233e+00 &                  8.459594e-01 &         1 \\
65  &    1717.212820 &              3.944939e+02 &              1.466371e+01 &         64.744883 &                   306.212357 &                    24.613384 &     0.050891 &                0.099732 &                0.009647 &  57645.423009 &             5.820766e-09 &             7.166818e-09 &         0.783199 &                8.441999e-02 &                1.778067e-01 &     0.561716 &                0.120901 &                0.204573 &         563.165645 &                  8.251099e+00 &                  5.248670e+00 &         1 \\
66  &    3140.121855 &              1.739853e+02 &              3.583373e+02 &        575.510591 &                    62.726776 &                    72.848583 &     3.561114 &                3.929403 &                2.090306 &  57645.424146 &             2.328306e-09 &             2.393790e-09 &         1.325460 &                1.263448e-01 &                1.174236e-01 &          NaN &                     NaN &                     NaN &         569.170711 &                  6.610805e-01 &                  7.126597e-01 &         1 \\
67  &    2440.903225 &              7.032350e+02 &              1.295474e+03 &       1928.192994 &                  1504.101602 &                  1071.471827 &     0.148669 &                0.065564 &                0.044160 &  57645.424618 &             3.557943e-09 &             8.018105e-09 &         0.724224 &                3.268988e-01 &                3.202378e-01 &     0.410055 &                0.248994 &                0.173052 &         564.742043 &                  7.263469e-01 &                  4.873390e-01 &         1 \\
68  &    3035.226950 &              2.527243e+02 &              6.986593e+02 &        579.911391 &                   121.772213 &                   164.150448 &     1.435790 &                2.901608 &                1.135001 &  57645.425478 &             9.131327e-09 &             7.596100e-09 &         1.023308 &                7.743977e-01 &                6.473015e-01 &     1.671389 &                0.886643 &                0.884146 &         563.240428 &                  2.225785e+00 &                  2.611995e+00 &         1 \\
69  &    1550.128232 &              1.061614e+01 &              1.094080e+01 &         76.312315 &                    10.644020 &                     9.747604 &     0.067294 &                0.008933 &                0.008195 &  57645.426792 &             8.440111e-09 &             6.293703e-09 &         0.611601 &                3.742269e-01 &                3.479874e-01 &     0.852257 &                0.338342 &                0.339446 &         562.579231 &                  1.106607e+00 &                  1.367854e+00 &         1 \\
70  &    1756.117968 &              4.413000e+02 &              5.008304e+01 &        192.621544 &                   198.203931 &                    46.269040 &     0.201899 &                0.384048 &                0.030120 &  57645.426923 &             3.739842e-09 &             3.361492e-09 &         1.386565 &                2.039221e-01 &                1.968113e-01 &     0.919056 &                0.300820 &                0.320082 &         571.125090 &                  9.088061e-01 &                  9.496840e-01 &         1 \\
71  &    1479.240651 &              8.003131e+00 &              7.914794e+00 &        119.941071 &                     7.755897 &                     7.230659 &     0.183004 &                0.010539 &                0.010273 &  57645.428905 &             5.697075e-09 &             5.777110e-09 &         2.410542 &                1.651075e-01 &                1.543151e-01 &          NaN &                     NaN &                     NaN &         569.043835 &                  7.462246e-01 &                  7.601764e-01 &         1 \\
72  &    1418.436500 &              4.440680e+01 &              4.953823e+02 &        118.600756 &                  2788.936113 &                    33.871782 &     0.087619 &                0.108905 &                0.017107 &  57645.429900 &             1.824810e-08 &             1.992885e-08 &         2.356641 &                6.131942e-01 &                5.952364e-01 &     0.784561 &                0.601771 &                0.306418 &         564.685902 &                  2.002196e+00 &                  1.993743e+00 &         1 \\
73  &    1476.162699 &              9.002641e+00 &              9.484050e+00 &         80.936688 &                     9.701613 &                     8.042037 &     0.123489 &                0.012649 &                0.012447 &  57645.430345 &             1.758599e-08 &             1.777516e-08 &         3.114675 &                4.073805e-01 &                3.695247e-01 &          NaN &                     NaN &                     NaN &         571.912940 &                  2.322698e+00 &                  2.465981e+00 &         1 \\
74  &    1721.339203 &              4.106734e+00 &              4.125865e+00 &         38.667816 &                     5.548194 &                     4.296246 &     0.171942 &                0.017513 &                0.016620 &  57645.430448 &             1.109584e-08 &             1.077569e-08 &         2.637024 &                8.387583e-01 &                6.512917e-01 &     3.353441 &                1.081659 &                1.138255 &         575.227980 &                  1.037588e+01 &                  9.917636e+00 &         1 \\
75  &    3086.667479 &              2.142312e+02 &              6.056490e+02 &        498.722282 &                    58.931269 &                   116.565989 &     6.516961 &                9.992173 &                5.509438 &  57645.431306 &             3.936293e-09 &             4.074536e-09 &         1.131361 &                1.734233e-01 &                1.837735e-01 &     0.587614 &                0.369326 &                0.275993 &         565.224818 &                  1.693125e+00 &                  3.897621e+00 &         1 \\
76  &    1692.871860 &              1.146298e+01 &              8.444990e+00 &         91.646632 &                    20.251070 &                    14.123113 &     0.095355 &                0.007254 &                0.006691 &  57645.431478 &             1.549779e-09 &             1.673470e-09 &         0.687566 &                7.854712e-02 &                7.777064e-02 &     0.219348 &                0.120278 &                0.082055 &         563.513258 &                  5.723842e-01 &                  5.491343e-01 &         1 \\
77  &    1561.692073 &              1.303021e+03 &              1.516138e+03 &       2832.011301 &                   831.532584 &                  1141.303726 &     0.201720 &                0.056948 &                0.052034 &  57645.432545 &             1.397711e-08 &             1.694571e-08 &         2.051485 &                8.049102e-01 &                8.878593e-01 &     0.915765 &                0.577661 &                0.343658 &         564.615438 &                  1.756645e+00 &                  1.456396e+00 &         1 \\
78  &    2886.980686 &              3.641469e+02 &              7.808702e+02 &        804.979024 &                   544.515982 &                   229.019999 &     0.280421 &                0.421296 &                0.137702 &  57645.433087 &             3.761670e-09 &             2.626621e-09 &         0.571785 &                3.737512e-01 &                3.931337e-01 &     0.963890 &                0.351383 &                0.383984 &         562.421584 &                  8.836179e-01 &                  5.134757e-01 &         1 \\
79  &    1667.327751 &              7.314304e+00 &              7.260931e+00 &         66.812593 &                     7.870246 &                     6.665671 &     0.093815 &                0.009607 &                0.008978 &  57645.434330 &             5.187758e-09 &             5.158654e-09 &         1.097623 &                2.287482e-01 &                2.309131e-01 &     0.703326 &                0.305770 &                0.306397 &         559.497769 &                  2.217240e+00 &                  2.023495e+00 &         1 \\
80  &    1601.963477 &              1.277694e+03 &              1.503042e+03 &       2819.214819 &                   836.621500 &                  1140.150497 &     0.131291 &                0.031019 &                0.030013 &  57645.440067 &             4.110916e-09 &             4.380126e-09 &         0.799775 &                2.307853e-01 &                2.377410e-01 &     0.299180 &                0.231177 &                0.122822 &         565.776251 &                  3.511802e-01 &                  3.632283e-01 &         1 \\
81  &    1687.768615 &              3.686276e+00 &              3.711556e+00 &         62.058151 &                     5.302570 &                     4.672710 &     0.154459 &                0.007777 &                0.007417 &  57645.440815 &             2.095476e-09 &             1.920853e-09 &         0.955599 &                1.111654e-01 &                1.192815e-01 &     0.481068 &                0.181199 &                0.188627 &         566.927119 &                  9.709680e-01 &                  1.006559e+00 &         1 \\
82  &    2012.812267 &              1.159713e+03 &              3.333432e+02 &        341.179486 &                   297.910241 &                   208.973441 &     0.244789 &                2.660051 &                0.134871 &  57645.442100 &             7.275958e-09 &             8.316420e-09 &         2.108279 &                4.172739e-01 &                3.788079e-01 &     0.825778 &                0.628305 &                0.367181 &         563.539968 &                  1.801948e+00 &                  2.112779e+00 &         1 \\
83  &    1469.085028 &              1.273257e+01 &              1.454663e+01 &         87.190691 &                    13.747526 &                    12.566362 &     0.084329 &                0.011578 &                0.010206 &  57645.442633 &             1.178705e-08 &             1.447188e-08 &         1.371368 &                3.061635e-01 &                3.487483e-01 &     0.647338 &                0.481793 &                0.291887 &         562.454932 &                  1.480708e+00 &                  1.395851e+00 &         1 \\
84  &    1671.039915 &              1.113620e+01 &              9.895401e+00 &        107.110278 &                    22.607508 &                    16.549133 &     0.095381 &                0.007534 &                0.006896 &  57645.444481 &             1.644366e-09 &             1.477019e-09 &         0.509815 &                1.027496e-01 &                8.774176e-02 &     0.459451 &                0.122129 &                0.134779 &         565.370224 &                  5.232001e-01 &                  4.982806e-01 &         1 \\
85  &    1480.346346 &              7.227445e+00 &              7.577572e+00 &         96.554595 &                    10.365147 &                     9.423247 &     0.161804 &                0.010538 &                0.010504 &  57645.444919 &             7.028575e-09 &             6.861228e-09 &         1.975454 &                2.235563e-01 &                2.246655e-01 &     0.517873 &                0.195281 &                0.147700 &         565.842807 &                  1.073413e+00 &                  1.137353e+00 &         1 \\
86  &    2780.502613 &              2.500543e+02 &              9.995685e+02 &        368.180339 &                    71.826952 &                   256.126994 &    10.415885 &               12.013203 &               10.275748 &  57645.445443 &             5.129550e-09 &             4.314643e-09 &         1.216438 &                2.802890e-01 &                2.696089e-01 &     0.872813 &                0.391531 &                0.373970 &         560.861657 &                  2.640700e+00 &                  2.211774e+00 &         1 \\
87  &    1487.773014 &              3.733883e+00 &              3.807171e+00 &         83.027930 &                     3.672020 &                     3.557013 &     0.141104 &                0.005723 &                0.005553 &  57645.448803 &             1.833541e-09 &             1.782610e-09 &         0.660208 &                3.446256e-02 &                3.341631e-02 &          NaN &                     NaN &                     NaN &         561.071367 &                  2.577523e-01 &                  2.595136e-01 &         1 \\
88  &    1460.096696 &              4.741149e+00 &              4.849608e+00 &         87.196937 &                     5.090963 &                     4.727356 &     0.236683 &                0.011926 &                0.011599 &  57645.449987 &             7.625204e-09 &             7.741619e-09 &         2.807350 &                1.910706e-01 &                1.701220e-01 &          NaN &                     NaN &                     NaN &         568.064149 &                  1.011289e+00 &                  1.005672e+00 &         1 \\
89  &    1468.658600 &              5.720229e+00 &              5.866068e+00 &         57.790404 &                     6.713271 &                     5.931767 &     0.109160 &                0.009557 &                0.008956 &  57645.451990 &             1.255103e-08 &             1.350418e-08 &         1.582808 &                2.202104e-01 &                2.275626e-01 &     0.451615 &                0.196799 &                0.145180 &         563.310760 &                  2.019741e+00 &                  1.876428e+00 &         1 \\
90  &    1441.750838 &              4.282132e+00 &              4.574567e+00 &         67.521331 &                     4.491711 &                     4.331328 &     0.142443 &                0.008169 &                0.007853 &  57645.453426 &             4.227331e-09 &             4.125468e-09 &         0.591629 &                8.301529e-02 &                7.364113e-02 &     0.396539 &                0.067631 &                0.063572 &         563.089528 &                  5.543240e-01 &                  5.741314e-01 &         1 \\
91  &    1699.312840 &              3.779977e+00 &              3.635988e+00 &         68.370255 &                     5.971942 &                     5.062319 &     0.286153 &                0.011905 &                0.011530 &  57645.453639 &             3.652531e-09 &             4.183676e-09 &         2.483659 &                1.467723e-01 &                1.608944e-01 &     0.630212 &                0.290123 &                0.196818 &         569.028554 &                  1.614829e+00 &                  1.599067e+00 &         1 \\
92  &    1569.933745 &              1.656213e+01 &              1.757871e+01 &        109.003850 &                    24.912993 &                    18.667109 &     0.072980 &                0.010282 &                0.010060 &  57645.453640 &             3.063178e-09 &             2.954039e-09 &         0.254396 &                1.648204e-01 &                1.264443e-01 &     1.411967 &                0.330369 &                0.274767 &         566.533113 &                  6.728565e-01 &                  7.640658e-01 &         1 \\
93  &    1725.024812 &              2.628075e+01 &              1.346705e+01 &         94.709930 &                    24.883944 &                    15.333299 &     0.186049 &                0.025653 &                0.018184 &  57645.454258 &             6.330083e-09 &             6.744813e-09 &         2.268887 &                3.416549e-01 &                3.406638e-01 &     0.905585 &                0.561563 &                0.394976 &         569.292928 &                  2.536592e+00 &                  2.556439e+00 &         1 \\
94  &    1576.744880 &              2.445421e+01 &              2.342648e+01 &        131.079919 &                    34.460174 &                    21.362071 &     0.100828 &                0.016266 &                0.013884 &  57645.457361 &             1.077569e-08 &             1.268927e-08 &         1.766544 &                8.953911e-01 &                7.852575e-01 &     1.844145 &                0.846138 &                0.810665 &         562.614312 &                  2.848020e+00 &                  2.809466e+00 &         1 \\
95  &    1577.552397 &              2.501565e+01 &              2.304966e+01 &        131.336004 &                    33.983069 &                    21.485348 &     0.101176 &                0.016160 &                0.013928 &  57645.457361 &             1.077569e-08 &             1.252920e-08 &         1.749081 &                9.040648e-01 &                7.903621e-01 &     1.846625 &                0.854186 &                0.816190 &         562.558001 &                  2.875217e+00 &                  2.784554e+00 &         1 \\
96  &    1667.386391 &              6.334383e+01 &              2.475809e+01 &        167.055473 &                    63.947137 &                    29.376005 &     0.205133 &                0.035931 &                0.021680 &  57645.458536 &             5.202310e-09 &             5.988113e-09 &         1.227376 &                3.951017e-01 &                3.237630e-01 &     2.575740 &                0.480812 &                0.453056 &         568.800809 &                  1.775660e+00 &                  1.623564e+00 &         1 \\
97  &    1685.621021 &              1.041330e+03 &              2.542183e+01 &        127.486496 &                   380.916953 &                    29.005063 &     0.093946 &                0.867994 &                0.012945 &  57645.459103 &             5.231414e-09 &             6.089977e-09 &         0.776975 &                2.793762e-01 &                4.525519e-01 &     1.165137 &                0.478490 &                0.433633 &         566.379933 &                  1.821465e+00 &                  1.802054e+00 &         1 \\
98  &    1404.767162 &              4.246737e+00 &              4.179313e+00 &         70.790571 &                     5.255382 &                     5.022942 &     0.219696 &                0.011578 &                0.010933 &  57645.462107 &             9.313226e-09 &             9.473297e-09 &         2.271639 &                2.147267e-01 &                2.379545e-01 &     0.538642 &                0.175217 &                0.134516 &         564.708325 &                  1.027707e+00 &                  1.050837e+00 &         1 \\
99  &    1564.161526 &              1.490550e+01 &              1.520809e+01 &        145.437862 &                    22.784740 &                    19.037722 &     0.093862 &                0.008250 &                0.007726 &  57645.464053 &             2.924935e-09 &             2.830348e-09 &         0.962076 &                1.890339e-01 &                1.963829e-01 &     0.451252 &                0.204958 &                0.185094 &         565.313351 &                  5.314845e-01 &                  5.523109e-01 &         1 \\
100 &    1595.749037 &              1.446407e+01 &              1.439002e+01 &        144.104436 &                    20.923474 &                    17.430612 &     0.121358 &                0.009528 &                0.008974 &  57645.464189 &             3.703462e-09 &             3.710738e-09 &         1.244406 &                2.045444e-01 &                1.971149e-01 &     0.676185 &                0.225945 &                0.226959 &         564.424909 &                  7.548122e-01 &                  7.685186e-01 &         1 \\
101 &    1595.063990 &              1.187663e+03 &              5.748560e+01 &        225.987576 &                  2384.186386 &                    92.760915 &     0.074805 &                0.127797 &                0.019338 &  57645.464504 &             4.802132e-09 &             6.883056e-09 &         0.898964 &                3.659809e-01 &                5.131654e-01 &     0.852086 &                0.559731 &                0.426303 &         567.123622 &                  1.694344e+00 &                  1.933640e+00 &         1 \\
102 &    1966.525128 &              1.061649e+03 &              9.618014e+02 &       1970.737810 &                  1485.777072 &                  1706.845842 &     0.187780 &                0.064073 &                0.107246 &  57645.465133 &             6.883056e-09 &             6.592018e-09 &         0.759331 &                3.598308e-01 &                3.950503e-01 &     1.244785 &                0.584390 &                0.528811 &         566.009529 &                  1.935865e+00 &                  7.164909e-01 &         1 \\
103 &    1480.411416 &              1.132439e+03 &              1.328713e+03 &       2685.980603 &                   940.372315 &                  1535.483238 &     0.249445 &                0.052931 &                0.089305 &  57645.466101 &             5.602487e-09 &             5.507900e-09 &         1.120910 &                2.250362e-01 &                2.290677e-01 &     0.853499 &                0.299941 &                0.270546 &         567.002550 &                  7.252529e-01 &                  9.279284e-01 &         1 \\
104 &    1707.801832 &              1.378613e+03 &              1.532414e+01 &         89.118709 &                   445.440501 &                    26.610952 &     0.105725 &                4.564796 &                0.015450 &  57645.466380 &             4.751200e-09 &             4.474714e-09 &         1.019786 &                3.128417e-01 &                2.776730e-01 &     1.281008 &                0.418171 &                0.443851 &         573.207006 &                  1.998230e+00 &                  3.367167e+00 &         1 \\
105 &    1901.548147 &              1.082015e+03 &              1.418163e+03 &       2541.995267 &                  1043.979742 &                  1358.104203 &     0.184137 &                0.048689 &                0.052797 &  57645.468339 &             9.880750e-09 &             1.043372e-08 &         1.383362 &                3.962387e-01 &                3.757498e-01 &     0.587090 &                0.361215 &                0.248660 &         565.521749 &                  1.024529e+00 &                  8.451510e-01 &         1 \\
106 &    1461.076106 &              1.262501e+01 &              1.295560e+01 &         85.245144 &                    11.894901 &                    10.166661 &     0.084625 &                0.011527 &                0.010755 &  57645.472362 &             1.103763e-08 &             9.844371e-09 &         1.110243 &                3.610032e-01 &                3.288853e-01 &     0.749826 &                0.341681 &                0.296195 &         563.598782 &                  1.437588e+00 &                  1.675788e+00 &         1 \\
107 &    1715.320616 &              7.813194e+01 &              1.576692e+01 &         95.379198 &                    69.513985 &                    20.686252 &     0.089624 &                0.032942 &                0.010734 &  57645.474139 &             2.663000e-09 &             2.604793e-09 &         0.690257 &                1.376523e-01 &                1.483729e-01 &     0.395660 &                0.193369 &                0.175950 &         561.227089 &                  1.142549e+00 &                  1.243536e+00 &         1 \\
108 &    1739.638221 &              1.846262e+02 &              4.982098e+01 &        229.296500 &                   107.793207 &                    42.555969 &     0.220687 &                0.104798 &                0.027413 &  57645.474448 &             3.637979e-09 &             3.630703e-09 &         1.703164 &                2.005568e-01 &                2.041107e-01 &     0.692113 &                0.267207 &                0.251620 &         570.610408 &                  7.343792e-01 &                  7.044133e-01 &         1 \\
109 &    1146.748385 &              3.366306e+02 &              1.402431e+03 &       1268.197550 &                  1953.434745 &                  1118.096950 &     0.086795 &                0.132006 &                0.043727 &  57644.409674 &             2.612069e-09 &             3.556488e-08 &         0.315255 &                1.403977e+00 &                1.723546e-01 &     0.312379 &                0.722624 &                0.137925 &         564.674681 &                  1.460324e+00 &                  4.092879e-01 &         1 \\
110 &    2944.173246 &              3.174336e+02 &              5.864031e+02 &        751.069969 &                   291.263416 &                   192.031255 &     0.570043 &                0.746781 &                0.291921 &  57644.409674 &             3.885361e-09 &             2.830348e-09 &         0.369395 &                2.490799e-01 &                2.281785e-01 &     1.314203 &                0.653280 &                0.679797 &         566.808964 &                  7.847368e-01 &                  8.769143e-01 &         2 \\
111 &    1417.185501 &              3.884362e+00 &              4.659306e+00 &        101.935080 &                     4.761585 &                     4.084079 &     0.325358 &                0.026361 &                0.022544 &  57644.411072 &             8.731149e-10 &             9.677024e-10 &         0.567630 &                2.700489e-02 &                2.445215e-02 &          NaN &                     NaN &                     NaN &         560.936842 &                  1.509793e-01 &                  1.044998e-01 &         1 \\
112 &    1393.269756 &              7.335915e+00 &              6.580718e+00 &        182.694545 &                     7.031695 &                     7.319653 &     0.467987 &                0.023566 &                0.028527 &  57644.411072 &             1.367880e-09 &             1.506123e-09 &         1.086188 &                3.465937e-02 &                3.873258e-02 &          NaN &                     NaN &                     NaN &         562.334956 &                  2.126868e-01 &                  1.065625e-01 &         2 \\
113 &    3075.140018 &              2.057216e+02 &              3.100464e+02 &        432.303770 &                    64.815598 &                    80.479943 &    13.452290 &               16.886532 &               10.182305 &  57644.412240 &             5.980837e-09 &             3.921741e-09 &         0.658892 &                3.373955e-01 &                3.599354e-01 &     0.768458 &                0.438102 &                0.388007 &         568.514000 &                  2.818942e+00 &                  2.877411e+00 &         1 \\
114 &    1463.742248 &              1.658431e+01 &              1.993333e+01 &         92.445449 &                    26.420576 &                    16.196889 &     0.088688 &                0.014082 &                0.013198 &  57644.412240 &             1.666194e-08 &             2.434535e-08 &         1.938207 &                8.501248e-01 &                9.716448e-01 &     1.217235 &                0.557406 &                0.491706 &         568.620714 &                  3.480267e+00 &                  2.489991e+00 &         2 \\
115 &    1571.805268 &              1.256349e+03 &              1.318236e+03 &       2666.550717 &                   958.678509 &                  1462.952833 &     0.123130 &                0.034537 &                0.042314 &  57644.418309 &             2.692104e-09 &             2.044544e-09 &         0.229590 &                1.847969e-01 &                1.297846e-01 &     0.668237 &                0.224315 &                0.184028 &         569.377581 &                  3.826299e-01 &                  5.025129e-01 &         1 \\
116 &    1545.045684 &              1.218522e+01 &              1.231491e+01 &         79.220876 &                    12.863110 &                    10.388883 &     0.070604 &                0.012331 &                0.009849 &  57644.418309 &             6.701157e-09 &             8.214556e-09 &         0.893852 &                2.734982e-01 &                3.360123e-01 &     0.801977 &                0.525646 &                0.426765 &         564.836206 &                  1.702351e+00 &                  1.442758e+00 &         2 \\
117 &    2930.107980 &              3.016985e+02 &              1.238434e+03 &        554.920581 &                  2490.569338 &                   124.141388 &     1.279397 &               14.634899 &                1.104360 &  57644.464507 &             4.205504e-09 &             1.034641e-08 &         0.439924 &                3.701301e-01 &                2.670467e-01 &     0.746212 &                0.558681 &                0.348719 &         565.336884 &                  3.505241e+00 &                  2.291546e+00 &         1 \\
118 &      42.021699 &              1.287440e+03 &              5.240128e+02 &        546.664913 &                   543.613741 &                   417.624036 &     0.680933 &               26.226319 &                0.604790 &  57644.464508 &             3.983223e-07 &             2.954766e-08 &         0.850994 &                3.160707e+00 &                5.917550e-01 &     0.739398 &                3.571361 &                0.399140 &         564.241525 &                  1.454247e+02 &                  1.787667e+02 &         2 \\
119 &    1662.786572 &              1.499023e+01 &              1.138795e+01 &        135.639202 &                    17.252011 &                    14.123430 &     0.489810 &                0.029315 &                0.025773 &  57644.464759 &             1.374428e-08 &             1.445005e-08 &         8.336477 &                4.778664e-01 &                5.268128e-01 &     2.020312 &                0.734084 &                0.560803 &         568.020948 &                  3.895079e+00 &                  3.654518e+00 &         1 \\
120 &    2408.606972 &              7.136065e+02 &              1.401466e+03 &       2188.401233 &                  1310.395809 &                  1218.531156 &     0.156516 &                0.046767 &                0.038592 &  57644.464760 &             1.382432e-09 &             1.200533e-09 &         0.185676 &                1.360711e-01 &                1.089510e-01 &     0.552460 &                0.157799 &                0.147933 &         561.288155 &                  2.687443e-01 &                  1.567342e-01 &         2 \\
121 &    2269.117500 &              9.391856e+02 &              6.164983e+02 &        480.669655 &                   257.208127 &                   340.492478 &     0.360950 &                1.617964 &                0.245056 &  57645.412282 &             4.707545e-09 &             7.203198e-09 &         0.923363 &                5.702387e-01 &                5.487713e-01 &     2.507109 &                0.622974 &                0.509643 &         561.226766 &                  2.176630e+00 &                  1.712408e+00 &         1 \\
122 &    2952.955595 &              2.777356e+02 &              9.628994e+02 &        444.308412 &                    83.254251 &                   219.514873 &     4.070263 &                6.121378 &                3.929537 &  57645.412282 &             4.198228e-09 &             4.321919e-09 &         0.806123 &                1.742116e-01 &                1.409412e-01 &     0.328451 &                0.252032 &                0.159700 &         566.470854 &                  1.882520e+00 &                  1.738781e+00 &         2 \\
123 &    1458.599318 &              1.644780e+01 &              1.490549e+01 &        129.153657 &                    20.637665 &                    18.109982 &     0.109650 &                0.011784 &                0.011503 &  57645.427339 &             9.611540e-09 &             8.738425e-09 &         2.425962 &                3.816166e-01 &                3.478435e-01 &          NaN &                     NaN &                     NaN &         561.417523 &                  1.233301e+00 &                  1.519567e+00 &         1 \\
124 &    1894.125125 &              1.118269e+03 &              1.280715e+03 &       2407.093455 &                  1151.324507 &                  1543.217255 &     0.170886 &                0.059182 &                0.063451 &  57645.427339 &             7.021299e-09 &             6.853952e-09 &         0.742815 &                4.118685e-01 &                3.354176e-01 &     0.999411 &                0.666392 &                0.459778 &         561.185124 &                  1.673829e+00 &                  3.835765e+00 &         2 \\
125 &    1619.393987 &              1.350507e+01 &              1.339468e+01 &        122.792391 &                    19.610028 &                    15.503931 &     0.125426 &                0.011404 &                0.010902 &  57645.430623 &             6.621121e-09 &             6.606570e-09 &         1.728894 &                2.681988e-01 &                2.719235e-01 &     0.833053 &                0.394873 &                0.348592 &         564.472772 &                  1.957007e+00 &                  1.993448e+00 &         1 \\
126 &    1591.185401 &              8.643409e+00 &              8.622450e+00 &        106.246000 &                     9.690033 &                     8.605795 &     0.125593 &                0.008276 &                0.008099 &  57645.430622 &             2.961315e-09 &             3.063178e-09 &         1.175100 &                1.450225e-01 &                1.730884e-01 &     0.425621 &                0.207728 &                0.160133 &         565.279441 &                  7.579312e-01 &                  8.540979e-01 &         2 \\
127 &    1321.229539 &              2.350287e+00 &              2.591631e+00 &        178.089922 &                     2.393557 &                     2.192153 &     1.727278 &                0.016501 &                0.015766 &  57645.460053 &             3.565219e-10 &             3.710738e-10 &         0.950290 &                1.873480e-02 &                1.945944e-02 &     0.359745 &                0.015174 &                0.014633 &         561.979243 &                  2.641728e-02 &                  2.541783e-02 &         1 \\
128 &    1612.124857 &              1.982065e+00 &              1.948663e+00 &         89.558102 &                     1.776238 &                     1.794595 &     0.394344 &                0.007414 &                0.007265 &  57645.460053 &             9.968062e-10 &             9.968062e-10 &         0.817610 &                3.670013e-02 &                3.776732e-02 &     0.246287 &                0.058706 &                0.065201 &         562.082991 &                  1.678879e-01 &                  1.549020e-01 &         2 \\
129 &    1180.703156 &              8.763004e+00 &              1.092836e+01 &         92.749644 &                     8.914158 &                     7.840191 &     0.347690 &                0.025733 &                0.022437 &  57645.460053 &             4.161848e-09 &             4.198228e-09 &         1.221049 &                8.947771e-02 &                7.062640e-02 &          NaN &                     NaN &                     NaN &         561.591314 &                  2.490463e-01 &                  2.528331e-01 &         3 \\
130 &    1510.117308 &              2.071554e+01 &              2.071554e+01 &        133.202939 &                    21.510060 &                    21.510060 &     0.042229 &                0.002325 &                0.002434 &  57645.442000 &             2.823072e-09 &             2.830348e-09 &         0.867898 &                2.088193e-02 &                2.088193e-02 &          NaN &                     NaN &                     NaN &           0.548700 &                  8.577100e-03 &                  8.577100e-03 &         1 \\
131 &    1670.266306 &              1.956107e+01 &              1.956107e+01 &         83.299578 &                    17.949689 &                    17.949689 &     0.038362 &                0.002933 &                0.004161 &  57644.430170 &             1.120497e-09 &             1.120497e-09 &         0.022502 &                5.245603e-02 &                5.245603e-02 &     1.184573 &                0.279687 &                0.279687 &         563.027933 &                  4.789163e-01 &                  4.789163e-01 &         1 \\
132 &    1597.958397 &              2.164807e+07 &              2.164807e+07 &        119.798457 &                815228.179720 &                815228.179720 &     0.046001 &              673.184372 &                     NaN &  57644.471178 &             1.926910e-02 &             1.926910e-02 &         0.000061 &                9.463654e+02 &                9.463654e+02 &     0.915043 &                0.194515 &                0.194515 &         564.219980 &                  1.263647e+06 &                  1.263647e+06 &         1 \\
133 &    1325.047334 &              2.504631e+01 &              2.504631e+01 &        155.341622 &                    23.929991 &                    23.929991 &     0.105346 &                0.009151 &                0.010004 &  57644.427210 &             1.682929e-08 &             1.682201e-08 &         1.862538 &                7.574584e-01 &                7.574584e-01 &     1.629269 &                0.519683 &                0.519683 &         563.619089 &                  1.438477e+00 &                  1.438477e+00 &         1 \\
134 &    1201.746909 &              9.566596e+00 &              9.566596e+00 &         50.113890 &                     9.582602 &                     9.582602 &     0.043276 &                0.002974 &                0.003165 &  57644.409568 &             1.412263e-08 &             1.411536e-08 &         1.352605 &                4.683643e-02 &                4.683643e-02 &          NaN &                     NaN &                     NaN &           0.914970 &                  1.221681e-01 &                  1.221681e-01 &         1 \\
135 &    1693.821972 &              1.558198e+01 &              1.558198e+01 &         87.565055 &                    17.957167 &                    17.957167 &     0.087618 &                0.007053 &                0.007637 &  57645.462556 &             6.097252e-09 &             6.104528e-09 &         1.141818 &                3.995876e-01 &                3.995876e-01 &     2.020600 &                0.633372 &                0.633372 &         567.138100 &                  2.866725e+00 &                  2.866725e+00 &         1 \\
136 &    1378.895119 &              1.347993e+00 &              1.347993e+00 &         30.835678 &                     1.344029 &                     1.344029 &     0.400891 &                0.010523 &                0.010797 &  57644.447727 &             1.723674e-08 &             1.722947e-08 &         0.783981 &                1.713189e-01 &                1.713189e-01 &     3.046816 &                0.209123 &                0.209123 &         558.887533 &                  1.729084e+00 &                  1.729084e+00 &         1 \\
137 &    1526.468893 &              2.556739e+01 &              2.556739e+01 &        136.077031 &                    27.045035 &                    27.045035 &     0.046438 &                0.003060 &                0.003225 &  57644.426304 &             4.481990e-09 &             4.474714e-09 &         1.484517 &                9.867641e-02 &                9.867641e-02 &          NaN &                     NaN &                     NaN &           0.942675 &                  3.104992e-03 &                  3.104992e-03 &         1 \\
138 &    1428.074624 &              1.130210e+01 &              1.130210e+01 &         75.406334 &                     9.214344 &                     9.214344 &     0.076461 &                0.001212 &                0.001677 &  57644.414472 &             1.908484e-08 &             1.908484e-08 &         1.978465 &                6.320594e-01 &                6.320594e-01 &     0.374386 &                0.569700 &                0.569700 &         564.319250 &                  2.101098e+00 &                  2.101098e+00 &         1 \\
139 &    1460.908407 &              6.399049e+01 &              6.399049e+01 &         93.404158 &                    18.294892 &                    18.294892 &     0.067000 &                0.073632 &                0.089068 &  57645.442741 &             1.317312e-07 &             1.317239e-07 &         0.007516 &                2.039446e+00 &                2.039446e+00 &     2.072048 &                0.536759 &                0.536759 &         568.595557 &                  7.617052e+00 &                  7.617052e+00 &         1 \\
140 &    1619.713506 &              1.240310e+01 &              1.240310e+01 &        103.789170 &                    13.706690 &                    13.706690 &     0.102777 &                0.006001 &                0.006370 &  57645.451201 &             7.850758e-09 &             7.843482e-09 &         1.720296 &                4.327078e-01 &                4.327078e-01 &     1.324193 &                0.543372 &                0.543372 &         561.153658 &                  1.922735e+00 &                  1.922735e+00 &         1 \\
141 &    1296.131947 &              2.760286e+01 &              2.760286e+01 &        144.063844 &                    25.669848 &                    25.669848 &     0.098513 &                0.011069 &                0.012383 &  57645.426747 &             1.644366e-09 &             1.637090e-09 &         0.014181 &                5.825055e-02 &                5.825055e-02 &     1.727077 &                0.438122 &                0.438122 &         566.064993 &                  1.382615e-01 &                  1.382615e-01 &         1 \\
142 &    1393.789741 &              1.799780e+06 &              1.799780e+06 &         52.886662 &                 34154.830232 &                 34154.830232 &     0.022488 &              397.050200 &                     NaN &  57645.426747 &             1.238509e-02 &             1.238509e-02 &         0.000018 &                1.200626e+06 &                1.200626e+06 &     1.195847 &                0.802779 &                0.802779 &         569.703900 &                  8.121671e+05 &                  8.121671e+05 &         2 \\
143 &    1475.052916 &              4.450116e+01 &              4.450116e+01 &        261.543218 &                    62.152991 &                    62.152991 &     0.075349 &                0.006574 &                0.007136 &  57645.454493 &             9.094947e-10 &             9.022187e-10 &         0.049879 &                6.966984e-02 &                6.966984e-02 &     1.394718 &                0.272584 &                0.272584 &         565.674154 &                  1.528706e-01 &                  1.528706e-01 &         1 \\
144 &    1558.745535 &              3.399751e+01 &              3.399751e+01 &        212.380150 &                    44.927400 &                    44.927400 &     0.089441 &                0.006933 &                0.007452 &  57644.408907 &             1.418812e-09 &             1.418812e-09 &         0.001231 &                1.571490e-02 &                1.571490e-02 &     1.947448 &                0.337326 &                0.337326 &         565.336150 &                  4.118707e-01 &                  4.118707e-01 &         1 \\
\enddata
\end{deluxetable*}


==> fitting_stuff.tex <==
check in final table: 
cand_tstart_57645.409861111111_tcand_1086.2000000_dm_562.05600_snr_6.40849_fit_results.png
cand_tstart_57644.407719907409_tcand_4864.6800000_dm_568.56200_snr_6.72464_fit_results.png
cand_tstart_57645.409861111111_tcand_159.4330000_dm_558.83100_snr_7.95436_fit_results.png

Good: 
1 comp:
cand_tstart_57645.409861111111_tcand_1719.8800000_dm_581.80000_snr_7.37079_fit_results.png
cand_tstart_57645.409861111111_tcand_3732.4400000_dm_565.30000_snr_6.74773_fit_results.png
cand_tstart_57645.409861111111_tcand_3589.8600000_dm_565.30000_snr_7.05175_fit_results.png
cand_tstart_57645.409861111111_tcand_965.5470000_dm_571.84300_snr_8.61639_fit_results.png
cand_tstart_57645.409861111111_tcand_644.5610000_dm_565.30000_snr_11.90090_fit_results.png

2 comp: 
cand_tstart_57645.409861111111_tcand_1743.9100000_dm_558.83100_snr_13.70630_fit_results.png


==> todo.tex <==
1. Introduction [KA, DA]
2. Data [KA, DA]
3. Methods 
4. Results
    - Burst Sample
        - Rerun Heimdall + Fetch [DA] 
            - Refer them to infinite freq, barycenter 
        - Get Burst TOAs [KA] https://iopscience.iop.org/article/10.3847/1538-4357/aaf6ef/pdf 
        - Calculate burst widths? [KA]
            - Simple widths reported by Heimdall OR
            - Fit the bursts with a template??? [optional] [KA]
        - Estimate burst flux [KA]
        - Estimate burst fluence [KA] 
        - Calculate Energy and luminosity of bursts []
    - Make burst energy distribution [Reshma]
        - estimate completeness, filter bursts above completeness
        - estimate gamma
    - DM analysis [optional] [KA]
        - str optimisind DM: https://github.com/danielemichilli/DM\_phase
        - Some discussion of sad trombone, sub burst drift rate, etc 
        
5. Discussion
    - Spectra 
        - Extract spectra of bursts
        - Fit spectra with a model (gaussian + a slope?) [optional]
    - Wait time [Evan] -- can use
        /hyrule/data/users/dagarwal/KG\_FRB121102/121102\_bursts.csv for now 
        - Use burst TOAs, get wait times
        - make wait time distribution
        - fit the distribution with something
    - Period search [Maura, Evan can help] -- can use
    /hyrule/data/users/dagarwal/KG\_FRB121102/121102\_bursts.csv for now 
        - Use techniques typically used for RRAT period searches
        - use frbpa
        - https://github.com/KshitijAggarwal/frbpa 
        - other methods?
        - https://github.com/evanocathain/Useful\_RRAT\_stuff/blob/master/getper.py 
    - burst rate? [Evan]
        - some discussion about this
        - Poisson vs Weibull: 
            - https://github.com/RuiLuoAstro/BayesWeib 
            - https://github.com/MJastro95/weibull\_analysis 
    - Progenitor models
        - need to do a quick literature review on FRB121102 theories
6. Conclusions

Tables:
1. Table with all burst properties: MJD, Width, Fluence, Freq bandwidth(?), DM

Figures: 
1. All Burst spectograms
2. Energy dist" 
3. Spectra (Update from fig 3 of Gourdji et al, to include actual burst spectras instead of just colored bands)
4. Wait time dist", with published points on it 
5. Peak of wait time dist" vs minimum energy burst used. Li et al says the wait time for all bursts is 70s while that of high energy bursts was 200. Maybe we can see something similar from this? 


Other: 
1. Maura to email Editor of APJ Letters to ask about page limits, etc 
2. DA to email all the authors of Gourdji et al 2019 and offering them to opt-in as co-authors.  

Relevant Links: 
https://ui.adsabs.harvard.edu/abs/2019ApJ...877L..19G/abstract
https://ui.adsabs.harvard.edu/abs/2021MNRAS.500..448C/abstract
https://arxiv.org/abs/2012.07303


Meeting: 
17 December: 
    1. Wait time: which log normal did they use, don't use the very small spacing bursts, mention the function in the paper, 
    2. Period: sim code by Maura, period diff code, Evan to try other techniques 
    3. Energy distribution: comparison with other papers. 
    4. Burst rate: only use bursts above completeness 
    5. nanograv does spectra temporal analysis code 
